Human Activity Recognition Based on Wearable Sensor Data: A Standardization of the State-of-the-Art

Human activity recognition based on wearable sensor data has been an attractive research topic due to its application in areas such as healthcare and smart environments. In this context, many works have presented remarkable results using accelerometer, gyroscope and magnetometer data to represent the activities categories. However, current studies do not consider important issues that lead to skewed results, making it hard to assess the quality of sensor-based human activity recognition and preventing a direct comparison of previous works. These issues include the samples generation processes and the validation protocols used. We emphasize that in other research areas, such as image classification and object detection, these issues are already well-defined, which brings more efforts towards the application. Inspired by this, we conduct an extensive set of experiments that analyze different sample generation processes and validation protocols to indicate the vulnerable points in human activity recognition based on wearable sensor data. For this purpose, we implement and evaluate several top-performance methods, ranging from handcrafted-based approaches to convolutional neural networks. According to our study, most of the experimental evaluations that are currently employed are not adequate to perform the activity recognition in the context of wearable sensor data, in which the recognition accuracy drops considerably when compared to an appropriate evaluation approach. To the best of our knowledge, this is the first study that tackles essential issues that compromise the understanding of the performance in human activity recognition based on wearable sensor data.

==> Figures/aan08060 <==
%PDF-1.5
%âãÏÓ
1 0 obj
<</Metadata 12 0 R/OCProperties<</D<</ON[13 0 R 29 0 R]/Order 30 0 R/RBGroups[]>>/OCGs[13 0 R 29 0 R]>>/Pages 3 0 R/Type/Catalog>>
endobj
12 0 obj
<</Length 18036/Subtype/XML/Type/Metadata>>stream
<?xpacket begin="" id="W5M0MpCehiHzreSzNTczkc9d"?>
<x:xmpmeta xmlns:x="adobe:ns:meta/" x:xmptk="Adobe XMP Core 5.3-c011 66.145661, 2012/02/06-14:56:27        ">
   <rdf:RDF xmlns:rdf="http://www.w3.org/1999/02/22-rdf-syntax-ns#">
      <rdf:Description rdf:about=""
            xmlns:pdf="http://ns.adobe.com/pdf/1.3/">
         <pdf:Producer>Artifex Ghostscript 8.54</pdf:Producer>
      </rdf:Description>
      <rdf:Description rdf:about=""
            xmlns:xmp="http://ns.adobe.com/xap/1.0/"
            xmlns:xmpGImg="http://ns.adobe.com/xap/1.0/g/img/">
         <xmp:ModifyDate>2018-03-21T11:22:03-03:00</xmp:ModifyDate>
         <xmp:CreateDate>2018-03-21T11:06:57</xmp:CreateDate>
         <xmp:CreatorTool>MATLAB, The MathWorks, Inc. Version 8.1.0.604 (R2013a). Operating System: Microsoft Windows 7.</xmp:CreatorTool>
         <xmp:MetadataDate>2018-03-21T11:22:03-03:00</xmp:MetadataDate>
         <xmp:Thumbnails>
            <rdf:Alt>
               <rdf:li rdf:parseType="Resource">
                  <xmpGImg:width>256</xmpGImg:width>
                  <xmpGImg:height>192</xmpGImg:height>
                  <xmpGImg:format>JPEG</xmpGImg:format>
                  <xmpGImg:image>/9j/4AAQSkZJRgABAgEASABIAAD/7QAsUGhvdG9zaG9wIDMuMAA4QklNA+0AAAAAABAASAAAAAEA&#xA;AQBIAAAAAQAB/+4ADkFkb2JlAGTAAAAAAf/bAIQABgQEBAUEBgUFBgkGBQYJCwgGBggLDAoKCwoK&#xA;DBAMDAwMDAwQDA4PEA8ODBMTFBQTExwbGxscHx8fHx8fHx8fHwEHBwcNDA0YEBAYGhURFRofHx8f&#xA;Hx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8f/8AAEQgAwAEAAwER&#xA;AAIRAQMRAf/EAaIAAAAHAQEBAQEAAAAAAAAAAAQFAwIGAQAHCAkKCwEAAgIDAQEBAQEAAAAAAAAA&#xA;AQACAwQFBgcICQoLEAACAQMDAgQCBgcDBAIGAnMBAgMRBAAFIRIxQVEGE2EicYEUMpGhBxWxQiPB&#xA;UtHhMxZi8CRygvElQzRTkqKyY3PCNUQnk6OzNhdUZHTD0uIIJoMJChgZhJRFRqS0VtNVKBry4/PE&#xA;1OT0ZXWFlaW1xdXl9WZ2hpamtsbW5vY3R1dnd4eXp7fH1+f3OEhYaHiImKi4yNjo+Ck5SVlpeYmZ&#xA;qbnJ2en5KjpKWmp6ipqqusra6voRAAICAQIDBQUEBQYECAMDbQEAAhEDBCESMUEFURNhIgZxgZEy&#xA;obHwFMHR4SNCFVJicvEzJDRDghaSUyWiY7LCB3PSNeJEgxdUkwgJChgZJjZFGidkdFU38qOzwygp&#xA;0+PzhJSktMTU5PRldYWVpbXF1eX1RlZmdoaWprbG1ub2R1dnd4eXp7fH1+f3OEhYaHiImKi4yNjo&#xA;+DlJWWl5iZmpucnZ6fkqOkpaanqKmqq6ytrq+v/aAAwDAQACEQMRAD8A9U4q7FXYq7FXYq7FXYq7&#xA;FXYq7FXYq7FXYq7FXYq7FXYq7FXYq7FXYq7FXYq7FXYq7FXYq7FXYq7FXYq7FXYq7FXYq7FUENZs&#xA;mZ1VZ29N2jYrbXBXkjcWowjo2/cYq3+lbX+S47/8e1x2/wCeeKuOq2u/wXG1f+Pa47f888VcdVtR&#xA;X4Ljb/l2uPCv++8Vd+lrWpHC42NP95rjwr/vvFXfpW1/kuP+ka48K/77xVw1a1JHwXG//LrceFf9&#xA;94q0NXtTT93c7062twOv/PPFXDV7QmgjuegO9rcj7VadY/b6MVb/AEra/wAlx2/49rjv/wA88Vd+&#xA;lbX+S47f8e1x3NP994q79K2v8lx/0jXHjT/feKu/S1rWnC47/wDHrcdjT/feKu/Str/Jcd/+Pa47&#xA;f888VcdVtd/guNq/8e1x2/554q46raivwXG3/LtceFf994q46tag04XHWm1tcHtX/feKu/Str/Jc&#xA;f9I1x4V/33irhq1qSPguN/8Al1uPCv8AvvFWhq9qafu7nenW1uB1/wCeeKu/S9pt+7ud6f8AHrc/&#xA;tdP91/f4Yq3+lbX+S47f8e1x3/554q79K2v8lx2/49rjuaf77xV36Vtf5Lj/AKRrjxp/vvFVk+t2&#xA;UEMk0iXAjjVnci1uDsnXYR4qj8VdirsVdirsVdirsVQelf7yv/zEXPj/AMtEnjiqMxV2KuxVav2n&#xA;+fv4Dx/hiq7FXYq7FVo/vG+Q8adT9GKrsVdirsVWn+8X5Hxp1H0YquxV2KuxVa32k+fv4Hw/jiq7&#xA;FXYq7FVsn2R816V8R4YquxV2KuxVB6z/AMce+/5h5elf5D4b4qjMVdirsVdirsVdirsVQOlOv1V9&#xA;j/vRddmPS5ceGKoz1FpWh2qfsn9nY9v9vFXGRRXY7VP2T2+jFXGRRXY7daKT0FfDFWlccnG+zU/a&#xA;P7IPh+r9eKsL/NHXfPGlabZyeUbF726kmK3KrbvOVj4VBoOm/fMTV5MkQOAWXofZ3SaPNkkNVLgi&#xA;I7erh3tlelXNxNptnJdo0d3LDE1whRl4yNGGcEEbUNf1ZkwJIF83SaiMY5JCG8RI17r2RIlU0oG3&#xA;pSqsOorvUbZJpaWVTIaBt1Q7hh9ommxFB037+PbFV3qLStDvQ/ZP7Ww7f7WKu9RfA9v2T3NPDFXe&#xA;ovgfD7J8aeGKsJ1T809MsPPtt5Qeyne6uGjQXSkCMGYAj4Duaf7WYk9WI5Bjrd6HT+zuTLopasSj&#xA;wxvbe9mbeotK0O1T9k/s7Ht/t5lvPOMiiux2qfsnt9GKuMiiux260UnoK+GKtO4DKN/tU/a/lJ7D&#xA;f/PvirfqL4Hw+yfCvhirhKpIFG32FVYdRXwxVoSqaUDb0pVWHUV3qNsVaaVSooG34EVDL9o7dvvH&#xA;34qu9RaVod6H7J/a2Hb/AGsVd6i+B7fsnuaeGKu9RfA+H2T408MVQetSKNHvjQ/7zzdmHRCOwriq&#xA;OxV2KuxV2KuxV2KuxVB6V/vK/wDzEXPev/HxJiqMxV2KuxVatOT/AD33r2Hbtiq7FXYq7FVop6jD&#xA;vQbV36nt2xVdirsVdiqDk0vS5L9LyS0ge8UVW4ZFMo40pQkV28a7ZHgF3W7cNRkEeASlw91mvkjM&#xA;k0uxV2KrWpyT57b07Ht3xVdirsVdiq2SnEV23XqePcdx/mcVXYq7FXYqg9Z/4499/wAw8vU0/YPf&#xA;tiqMxV2KuxV2KuxV2KuxVA6S5Nq54k/6RddCD0uXHtiqM5NT7B77bdunfvirizb/AAE0r4b0+nvi&#xA;rizCvwE06UpvtXxxVarkvIKV4tTZgf2AdxtT5fTiq7k38h/Dwr4/Rirg7Ej92wr1J47bV8foxVoS&#xA;MaVjYVpWvHao70PbFVqSsZSpQj4EYjkpI5Fq1UHtTr3+jFV/JqfYPbbbv179sVdyb+Q9vDuaePbF&#xA;Xcm/kP4eNPH6cVWmRhKo49Vc05CuxUfZ79evbFXn35dfl55h8sa/qmo6jqIvoL1HWGFWclD6vMfb&#xA;NNxmDpdLLHIkm7ep7c7cwavBDHjhwShzO2+1dHoZZt/gJpXw3p9PfM55ZxZhX4CadKU32r44qtkc&#xA;h0FOrEfaAr8BOw7/AC+nFV3Jv5D+HhXx+jFXB2JH7thXqTx22r4/RirQkY0rGwrSteO1R3oe2KrX&#xA;lbipKFKlKlmUU5NQioJ3H44qv5NT7B7bbd+vftiruTfyHt4dzTx7Yq7k38h/Dxp4/TiqC1uRl0a/&#xA;PE7W0x3IUbIe9dq9cVR+KuxV2KuxV2KuxV2KoLSDW1k3r/pN0OtelxJiqNxV2KuxVZGatIK1o1KV&#xA;Bp8INPbFV+KuxV2KrAf3zCvRVPGo2qW3piqhqGraXpqLJqF5BZxueKPcSJEGPWgLkVORlOMeZpuw&#xA;6bJlNY4ymR3An7kRHJHLGskbB43AZHUgqVIqCCOoOSBapRINHmuxQhri+s7e4jjnuY4XdW4I8iqW&#xA;3A2U7nAZAc2yGGchcQSPcicLW7FXYqskNGjFaValKgV+Emnviq/FXYq7FVkpooNafEorUDqwFN/H&#xA;FV+KuxV2KoLWzTRr81pS2mNa0p8B7npiqNxV2KuxV2KuxV2KuxVA6S7fVX+Fm/0i67r2uXHY/wCf&#xA;ffFUZyan2D3227dO/fFXFm3+AmlfDen098VcWYV+AmnSlN9q+OKrVducgozUag3XYcAdqb9fHf6M&#xA;VXcm/kP4eFfH6MVcHYkfu2FepPHbavj9GKtCRjSsbCtK147VHeh7YqtSRzKQUYDgh4kpsWLV6GtR&#xA;Tft4d8VY5568g6R50srW01R7qCO1k9aM2zxK3JhxIbmsg2HhmPqNNHKAJXs7fsftrNoJyliESZCv&#xA;Vf6CE/sLVLKxt7OIOYraKOGNnKliqAICaUFaCp2y+MaADrM2U5JmZ5yJPzV+TfyH8PGnj9OFrYJ5&#xA;8/LC18267pupTXktq9ghCxIiMG4Sh96sDvyzD1GjGWQldU9H2P7RT0OGeIQEuPz8qZfrGtado2nT&#xA;alqcv1aygp6szbheThF6V+0zCn45kzmIizydHpdLkz5BjxjimeQ927tI1rTtY06LUtMl+tWM3P0Z&#xA;02VvTYoacqH7SkfRjCYkLHJdVpcmDIceQcMxzHv3RhZhX4CadKU32r45NoWyOwdAA27EbFdxwJ77&#xA;9fDf6MVXcm/kP4eFfH6MVcHYkfu2FepPHbavj9GKtCRjSsbCtK147VHeh7YqteR+K/AyVKVNU25N&#xA;uNyenf8ADFV/JqfYPbbbv179sVdyb+Q9vDuaePbFXcm/kP4eNPH6cVQetuw0a/IVqi2m3BUHZD4m&#xA;nvv9OKo7FXYq7FXYq7FXYq7FUHpX+8r/APMRc+H/AC0SeGKozFXYq7FVq/af5+3gPD+OKrsVdirs&#xA;VWj+8b5Dwp1P04quxVgP5ueR5vNVhp6R6rDpQtJXZpZyQr+ooAUEFd/hzC1un8QDeqem9mu1xo5z&#xA;JxnJxAculM20+IQ2FtCJBKI4kQSjo3FQOQ69cy4igHns8uKcjVWSrH+8X5Hwp1H05JqS7zN5d07z&#xA;Holzo2o8/qd1w9X0m4v+7kWRaGh/aQZXlxDJExPIuZoNdk0uaObHXHG6vzBH6XeWfLuneXNEttG0&#xA;7n9Ttefpeq3J/wB5I0jVNB+05xxYhjiIjkF1+uyarNLNkrjlV15AD9CZ5Y4a1vtJ8/bwPj/DFV2K&#xA;uxV2KrZPsj5r0p4jxxVdirsVdiqD1n/jj33/ADDy9KfyHx2xVGYq7FXYq7FXYq7FXYqgtL9QWr/C&#xA;P96Lrqf+Xh6dB4Yqi6yU2UV3puevbt3xVxMm9FHem569u2KuJk3ooPhUkdvl44q0PUDP8OxbapHT&#xA;iN9h4+OKt1k/lH3npT5eOKuBlqKqoHejE7U+XjirQM21VUdOVGJptvT4cVaX1udWUCqrUhqiu/ID&#xA;YHbFV1ZKbqK7V3PXv27Yqxf8xPIsfnXRINKuLk2aQ3KXQljAckqkkZWh49pK5j6nTjLHhJrd3PYf&#xA;bEuz8xyxjx3Hh7uoP6E90iwbTdJstOUiRbKCK3WQmhYRKE5EU7gVy6EeGIHc63U5/FyyyEVxyJ+Z&#xA;tFH1OYPEdG77dRTtXpkmhuslNlFd6bnr27d8VcTJvRR3puevbtiqjfXsVjZ3F7cssVraxvNNKxNF&#xA;jjXkzGgPShwSkALPJsxYpZJiERcpEADzPJB6J5i0nX7T67o1yl7aJK0RmjqAGVKkHkoP7Q6ZDHlj&#xA;MXE2G7WaHNpp8GWPDKrryTKsn8o+89KfLxyxxXAy1FVUDvRidqfLxxVoGbaqqOnKjE023p8OKtH1&#xA;iBVR+wTxau9fi6joMVXVkpuortXc9e/btirqyfyjt3Pjv28MVdWT+Ufeelfl4Yqg9a9X9D31FBP1&#xA;ebav+QadRTpiqOxV2KuxV2KuxV2KuxVB6UKWr7U/0i58P+WiTwxVGYq7FXYqtUUZ9qVNa7b7DwxV&#xA;dirsVYv+YreeV0GM+S0D6v8AWE5hvQp6HF+X+9BCfa4++Y+p8Th/d/V+O93PYY0Zzn85/dcJ/nfV&#xA;tX0796caB+lP0PYNqy01U2kH6Qpw/wB6OH70VjPHZ69NvDLcd8I4udbuv1nh+NPwv7vilw8/pvbn&#xA;vy790wybjOxV2KrSP3imnQEV27kfTiq7FVGG+sp5WihuI5ZUrzjR1ZloaGoBqN8AkC2SwziLIIB8&#xA;lPVdOt9T0y80255fVr2CS2n4GjcJUKNQ70NGwTiJAg9WWnzyw5I5I/VCQkPeDaWeUvJ2keVNM/Rm&#xA;kiQ2rTtcH1mDsHdAp3ou3wjK8OCOONRcvtPtTLrcviZa4qrbb8c09y51zsVdiq2QVUbV3U02PQjx&#xA;xVdirsVdiqD1kV0e+FK1t5dtj+wfHFUZirsVdirsVdirsVdiqB0r1BavRV/3ouvb/j5enY9RiqMr&#xA;JTZRXem569u3fFXEyb0Ud6bnr27Yq890j8uvMVj+ZV55ql1KOXTZ2naOw5S8h6q0UEEcNjmDDSyG&#xA;Yzvbuep1XbmDJ2fHTCFZI8Pq26fa9BXmGeiru2x6VHEbnbffbM55Zusn8o+89KfLxxVwMtRVVA70&#xA;Ynany8cVaBm2qqjpyoxNNt6fDirS+r6hLIoqqVIJrWrchWm4HbFV1ZKbqK7V3PXv27Yq6sn8o7dz&#xA;479vDFXVk/lH3npX5eGKrT6nqKeK9G338RTencdcVXVkpsorvTc9e3bvirBvJf5WW/lbzLqWuQXz&#xA;3T6ikqmB1CBfUlWUfEK/y0zDwaMY5mV83o+1vaKes08MJgIiFb3zoUzkmTeig+FSR2+XjmY840/P&#xA;ktFU0bYnw4nfptvtirdZP5R956U+XjirgZaiqqB3oxO1Pl44q0DNtVVHTlRiabb0+HFWm9UqOSL+&#xA;wTuWoa/F2HTscVXVkpuortXc9e/btirqyfyjt3Pjv28MVdWT+Ufeelfl4Yqg9a9T9D31FUn6vNsS&#xA;SPsGm1O4xVHYq7FXYq7FXYq7FXYqg9K/3lf/AJiLntT/AI+JMVRmKuxV2KrVpyf577U7Dv3xVdir&#xA;sVdiq0U9Rj3oN6b9T374quxV2KuxVaaeop70O9N+o79sVXYq7FXYqtanJPnttXse/bFV2KuxV2Kr&#xA;ZKcRXfdeo5dx2H+YxVdirsVdiqD1n/jj33/MPL1Ff2D274qjMVdirsVdirsVdirsVQOlc/qr0A/3&#xA;ouu5H/Hy9OoxVGVkpsorvTc9e3bviriZN6KO9Nz17dsVcTJvRQfCpI7fLxxVpefJ6Afa9xtxHt4+&#xA;GKt1k/lH3npT5eOKuBlqKqoHejE7U+XjirQM21VUdOVGJptvT4cVaUy+oeSqPhStCetWrvShp2xV&#xA;dWSm6iu1dz179u2KurJ/KO3c+O/bwxV5X5G/MPzLZ391p/5jzR6dez/Vv0RBJGsbSCR5EkI9IN3C&#xA;/azW6fUzBIy7HantO2OxNPkhHJ2eDkgOLjN3VcJHP4pr+a35fa/5wOlDS9QTTzZC59bk0oDiUxcd&#xA;4x29M9ct1mmllrhNU4Xs523h0PieLAz4+GuW1cXf72f1kpsorvTc9e3bvma8w4mTeijvTc9e3bFW&#xA;Dah+bui2X5mWv5fvZ3Daldxhku1C+iGaMyorb89wpqQNvvpvMXYOWeilqwY8ETy6869zUco4uFnD&#xA;8+S0A+1t16cT4DbfNG2sCj/MvVn/ADfl8ifoKUWEdqJxrFX4lvRE3L7HH0+TelWv2/uzfHseA7OG&#xA;q8QcZlXB8a7+f8XuavEPHw0mtn+Zvla788XHkmG45a7apzmiCv6eyB3VZOPEsoYVH8RTMXJ2PqIa&#xA;Uakj91I9+/yZDIOLh6soBm2qqjpyoxNNt6fDmrZtMZSo5Ko+xWhLb136AdOxxVdWSm6iu1dz179u&#xA;2KurJ/KO3c+O/bwxV1ZP5R956V+XhiqD1oyfoe+oo/3nm7k/sGnQV6YqjsVdirsVdirsVdirsVQe&#xA;lf7yv/zEXPj/AMtEnjiqMxV2KuxVav2n+fv4Dx/hiq7FXYq7FVo/vG+Q8adT9GKrsVdirFvM35be&#xA;W/Mmt2Ws6kJzeWCosHpycEpHIZByFDX4jmNl0sMkhI8w7ns/t7UaTDLDj4eCd3Y7xTJz/eL8j406&#xA;j6MyXTLsVef+RPzXfzX5x8w+XDodzpw0JmUXkzVEnGT06OnBfTZvtKOTVGb/ALT7D/K6bFm8SM/F&#xA;6DptfO9+48mqGXiJFcmctYWL3iXzW0TXsamOO6KKZVQ1qoenIDfpXNIMshHhs8Pd0+TZSq32k+fv&#xA;4Hw/jlaV2KpPD5P8rw+Y5fMsWmQJrs0fpS6gEpKy0A69K0AFetNszJa/OcIwmZ8IG+Hox4Bd9U4z&#xA;DZLZPsj5r0r4jwxVdirsVdiqD1n/AI499/zDy9K/yHw3xVGYq7FXYq7FXYq7FXYqgdK5/VXoR/vR&#xA;ddif+Pl6dTiqMpJTZhXemx69u/bFXESb0Yd6bHr274q4iTejAeFQT2+fjirS8+T0I+17nbiPfx8M&#xA;VbpJ/MPuPSnz8cVcBLUVZSO9FI2p8/HFWgJtqsp6cqKRXbenxYq0ol9Q8mU/ClaA9atXatBXtiq6&#xA;klN2Fdq7Hr3798VdST+Ydux8d+/hirqSfzD7j0r8/DFWAeb9I/Me58/6Ld6JdtF5dh+rfpKFZhGr&#xA;BLlmmrGTVv3JUHxzCzQynLExPo2v5vT9manQQ0OWGaIOoPHwHhv+EcO/9Zn9JKbMK702PXt37Zmv&#xA;MLJ5RBDLPLIqRRIzu5BooUVqd+wG+SjEyIA5lWOeRvzF8s+eLO7u/L1y00VnMYJhLE0bAkVRqMRV&#xA;W6j+BzY9p9kZ9FIRzCjIWN7YQyCXJkr8+S0I+1t16cT4HffNYzbpJ/MPuPSnz8cVcBLUVZSO9FI2&#xA;p8/HFWgJtqsp6cqKRXbenxYq0wlCjkyn7FaArvXfoT17DFV1JKbsK7V2PXv374q6kn8w7dj479/D&#xA;FXUk/mH3HpX5+GKoPWhJ+h76jD/eebsR+wadDXpiqOxV2KuxV2KuxV2KuxVB6V/vK/8AzEXPev8A&#xA;x8SYqjMVdirsVWrTk/z33r2Hbtiq7FXYq7FVop6jDvQbV36nt2xVdirsVdiq009RR3odq79R274q&#xA;uxVplV1KsAysKMp3BB7HCDSpT5b8o+WvLNtLa6Bp0OnQTyGaZIVpycilSTU9Og7ZlazX5tTISyyM&#xA;yBW7GMQOSatTknz23p2PbvmIyXYq7FXYqtkpxFdt16nj3Hcf5nFV2KuxV2KoPWf+OPff8w8vU0/Y&#xA;PftiqMxV2KuxV2KuxV2KuxVA6T6htXoy/wC9F0Nvi/4+Xp3HQdcVRlJKbMK702PXt37Yq4iTejDv&#xA;TY9e3fFXESb0YDwqCe3z8cVWqXLyAMuzUA6kDgNj0oa7/LFV1JP5h9x6U+fjirgJairKR3opG1Pn&#xA;44q0BNtVlPTlRSK7b0+LFVqer6pVnQ0RKgVrWrcjxrsD2xVfSSm7Cu1dj179++KupJ/MO3Y+O/fw&#xA;xV1JP5h9x6V+fhiqX6rrmk6VJbDVNStLAXTNFbi6mSEyyVXikYdl5mnhl+HTZct+HGUuHc0Ca99I&#xA;MgOaYUkpswrvTY9e3ftlCWBfmp+bEX5fvoyS6ZNqR1maSFPQ+H0/T4eNebn1PhTblvuKZvuxOwpa&#xA;8ZKmIeGL363f2bblqyZeGmeSCYq3BgCQeFR0NNvxzRBteG/843+X/O3lzSvMknmGwvLZ5bpJLeC6&#xA;YmSd44pTJ6SNuzMePxdG+jO29sNXptRkwjDKB9O5HS6q/t26ONp4kA2zf8ovzI1bz3pWoXl/oz6M&#xA;9ldG3VX5ssg41oCyxnmh2fNL292RDQ5IxhkGTijfu+07Ho2YshkOTPAJairKR3opG1Pn45om1oCb&#xA;arKenKikV23p8WKvMf8AnIHz7rHk7yZBPpGpRWGs3lzHFbyND6hZUBaYqHWVB+z9odK96Z03sr2X&#xA;j1mpIyxM8cY2d636dQfk055mI25s28l3er3nlPSLvVbi3udSntIXu57WjQvIVBdlKnjv/k7V6bbZ&#xA;pu0ceOGonHGDGAkaB502QJoWnNJP5h27Hx37+GYTJ1JP5h9x6V+fhiqC1v1Bo1+Qygi2mNTUAfAa&#xA;VNdqDriqPxV2KuxV2KuxV2KuxVBaQa2sm9f9Juh1r0uJMVRuKuxV2KrIzVpBWtGpSoNPhBp7Yqvx&#xA;V2KuxVYD++YV6Kp41G1S29MVX4q7FXYqw38wfyu8q+e7jSv08JydKaWW2WCUR8hIY/UVwVYlT6a1&#xA;pQjx3zb9ldt59CJ+FX7wC7F8rqvm1zxiXNmWahscQDQkVpuPbtirsVWSGjRitKtSlQK/CTT3xVfi&#xA;rxT/AJyl1iOPytpPl6S0u5l1u8H+kWrACM25T4XQq3ql/V+FKrUitds7T2K05OeeYSiPDjyl1u/l&#xA;VbnfnycfUnYDveseWNDTQPLunaLHcS3Sadbx2y3E5rI4jUKCf4DsNs5TW6k580spAjxyJoct26Io&#xA;UwH8+/IOuedND0+w0uKKQQzO8zStGhUsAqFGfcGu23XBpO1NVos0cunP9YHlIdx/Gzuuyo6CUckd&#xA;XYsDhIuwe/8AtZb+Xfky18m+T9P8v20kkq2qs0skrciZZWMklKfCF5MaAfrqcv7T7RnrM5zTAEpV&#xA;sPIU6fgjHaO4ZJmArAo/ynt0/NuX8xf0pMZpIBD+jOI9MUgEH2+VeNF5ceP2t65vj24T2eNHwCgb&#xA;4uv1cXL7L7mrwvXxMw1s00a/NaUtpjWtKfAe56ZoW1G4q7FXYq7FXYq7FXYqgdKDG1f4z/vRdD9k&#xA;/wDHy/gO3T9e+Kozi1Ptnvvt36du2KuKtv8AGRWvhtX6O2KuKsa/GRXpSm21PDFVqhi0nxnZth8O&#xA;w4DbYfTvv9GKruLfzn8PCnh9OKuCMCP3jGnUHjvtTw+nFWhGwpWRjSla8d6DvQd8VWoriUgyMwCJ&#xA;seHWrVOwrVu/bw74qv4tT7Z7b7duvbviruLfznt4djXw74q7i385/Dxr4fRiq0hvVUeowBVjT4fF&#xA;adq7dP19sVXcWp9s999u/Tt2xVg3mv8AOLyVoWka9eQ6jHqN9oI9O5023dfV9eRxFGlSpAAk+Fm3&#xA;49wTtm80Xs/qs+THExMI5eUjyrmT8uQ6tUssQD5In8qfPN7558mweYLqxbTJJ5ZYliDc0cRnj6kT&#xA;MoJWtRv+0CMr7c7MjotScMZcdAH3X0KcU+IWy6QNySjkVY7Dj04HbcfTtv8ARmnbF3Fv5z+HhTw+&#xA;nFWD/mn+VGn/AJh6dYWV9qNxZCwn9dHhCMG5JxYFSBv4Htvm77D7cn2fOUoxEuIVu15MfGzO1tBb&#xA;W8MCSuyQokalyCSEXj8RpuT3zTTkZEk9Wxc6uqqfVbYoD9gV+Kh6j9qu/wCFMiq/i1Ptntvt269u&#xA;+Ku4t/Oe3h2NfDviruLfzn8PGvh9GKoPW1YaNfkSMCLebcca/YJ7im3v9OKo7FXYq7FXYq7FXYq7&#xA;FUHpX+8r/wDMRc+H/LRJ4YqjMVdirsVWr9p/n7eA8P44quxV2KuxVaP7xvkPCnU/Tiq7FXYq7FVp&#xA;/vF+R8KdR9OKrsVYbo/5Q/l/pWp6zqNvpUcsmvVGoQXP7+AqziVkWKTkgVpAGpTr0oM3Go7e1eWG&#xA;OBmQMX0kbHlXMb8tmsYognzZZZ2dnZWsVpZwR21rAoSG3hRY40UdFVFAVQPAZqsmSU5GUiTI8ydy&#xA;2AKjfaT5+3gfH+GQVdirsVdiq2T7I+a9KeI8cVXYq7FXYqg9Z/4499/zDy9KfyHx2xVGYq7FXYq7&#xA;FXYq7FXYqltto01sJVi1K64STTThCLchDPI0rKp9GvEFiBUk074qrfUbr/q43Hf9m37/APPLtirj&#xA;Y3W/+5G47/s2/f8A55dsVcbG6Nf9yNwK/wCTb7bf8YsVd9Quak/pG43Nfs2/hSn919OKu+o3X/Vx&#xA;uP8Agbfwp/vr6cVcLC6BH+5K4NP8m332p/vn6cVaFhdCn+5K5NKdVt96f88e+KuGn3QNf0lcHYA1&#xA;W27V32h71xVv6jdf9XG47fs2/b/nl3xV31G6/wCrjcdv2bfsf+MWKu+o3X/VxuP+Bt/Gv++voxVo&#xA;6fdVB/SNxsCPs2/cg/757UxVv6jdf9XG47/s2/f/AJ5dsVcbG63/ANyNx3/Zt+//ADy7Yq42N0a/&#xA;7kbgV/ybfbb/AIxYq42FySD+kbgUNfs2/hSm8X04q76jdf8AVxuP+Bt/Cn++vpxVwsLoEf7krg0/&#xA;ybffan++fpxVoWF0Kf7krk0p1W33p/zx74q79H3VADqVyacf2bbfia/7574q39Ruv+rjcdv2bft/&#xA;zy74q76jdf8AVxuO37Nv2P8AxixV31G6/wCrjcf8Db+Nf99fRiqje6NLeWc9pLqNyIriN4pCotw3&#xA;GQUND6PUA7YqmWKuxV2KuxV2KuxV2KuxV2KuxV2KuxV2KuxV2KuxV2KuxV2KuxV2KuxV2KuxV2Ku&#xA;xV2KuxV2KuxV2KuxV2KuxV2KuxV2KuxV2KuxV2KuxV2KuxV2KuxV2KuxV2KuxV2KuxV2KuxV2Kux&#xA;V2KuxV2KuxV2KuxV2KuxV2KuxV2Kv//Z</xmpGImg:image>
               </rdf:li>
            </rdf:Alt>
         </xmp:Thumbnails>
      </rdf:Description>
      <rdf:Description rdf:about=""
            xmlns:xmpMM="http://ns.adobe.com/xap/1.0/mm/">
         <xmpMM:DocumentID>9d9ca01c-2f6c-11e8-0000-abebf2b7c7af</xmpMM:DocumentID>
         <xmpMM:InstanceID>uuid:2c50a6ff-eed6-4833-8d18-2c6d2bf69159</xmpMM:InstanceID>
         <xmpMM:RenditionClass>proof:pdf</xmpMM:RenditionClass>
      </rdf:Description>
      <rdf:Description rdf:about=""
            xmlns:dc="http://purl.org/dc/elements/1.1/">
         <dc:format>application/pdf</dc:format>
         <dc:title>
            <rdf:Alt>
               <rdf:li xml:lang="x-default">C:\Users\ARTUR\AppData\Local\Temp\tp4792015e_cbd9_429d_9b9c_601433acb843.ps</rdf:li>
            </rdf:Alt>
         </dc:title>
      </rdf:Description>
      <rdf:Description rdf:about=""
            xmlns:xmpTPg="http://ns.adobe.com/xap/1.0/t/pg/"
            xmlns:stDim="http://ns.adobe.com/xap/1.0/sType/Dimensions#"
            xmlns:xmpG="http://ns.adobe.com/xap/1.0/g/">
         <xmpTPg:NPages>1</xmpTPg:NPages>
         <xmpTPg:HasVisibleTransparency>False</xmpTPg:HasVisibleTransparency>
         <xmpTPg:HasVisibleOverprint>False</xmpTPg:HasVisibleOverprint>
         <xmpTPg:MaxPageSize rdf:parseType="Resource">
            <stDim:w>325.500977</stDim:w>
            <stDim:h>257.917969</stDim:h>
            <stDim:unit>Points</stDim:unit>
         </xmpTPg:MaxPageSize>
         <xmpTPg:PlateNames>
            <rdf:Seq>
               <rdf:li>Cyan</rdf:li>
               <rdf:li>Magenta</rdf:li>
               <rdf:li>Yellow</rdf:li>
               <rdf:li>Black</rdf:li>
            </rdf:Seq>
         </xmpTPg:PlateNames>
         <xmpTPg:SwatchGroups>
            <rdf:Seq>
               <rdf:li rdf:parseType="Resource">
                  <xmpG:groupName>Default Swatch Group</xmpG:groupName>
                  <xmpG:groupType>0</xmpG:groupType>
               </rdf:li>
            </rdf:Seq>
         </xmpTPg:SwatchGroups>
      </rdf:Description>
   </rdf:RDF>
</x:xmpmeta>
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                           
<?xpacket end="w"?>
endstream
endobj
3 0 obj
<</Count 1/Kids[4 0 R]/Type/Pages>>
endobj
4 0 obj
<</ArtBox[0.0 0.0 325.501 257.918]/BleedBox[0.0 0.0 325.501 257.918]/Contents 31 0 R/LastModified(D:20180321112203-02'00')/MediaBox[0.0 0.0 325.501 257.918]/Parent 3 0 R/PieceInfo<</Illustrator 32 0 R>>/Resources<</ExtGState<</GS0 33 0 R>>/Properties<</MC0 29 0 R>>>>/Rotate 0/Thumb 34 0 R/TrimBox[0.0 0.0 325.501 257.918]/Type/Page>>
endobj
31 0 obj
<</Filter/FlateDecode/Length 827>>stream
H‰ÌWËnÛ0¼ë+x.`…Ë7¯qŸ'Â塇 §4
$'úû].-™¢$GBƒPp`EäÎpøØåøêëž]Ýì9»þ¼gÍKÙжõà˜ºÕØ®kx½o¾³ß
°CÃ[Íþ2`¬¹:ÎþÐ ¦ì0)%o#^ýàì'ÃvΞ3ôƾ ulß]ûÝsÊ)èxR'Ek…,0ç< …çº9˜.¼d™F※Ëꆡï>¼­Õ‹¤è÷!À -,Uх¿»ËWÉ8…ÿ·Œtú2æ.ô'¨K©AïgúaVMÛO%O>Ó
}ò§$
Ó¬h9WЖˆi^kqðU¼%bš¸X+x™an­äd†Y«áÙXÀ\Bf˜oùJæ2sÚ¸^«y™a–°Vó2Ã\æàæ·n´ÛüfòMՈ®MƊ½ Ñû¸¾LŒ
ÄÔ¼z'Ç&…½>œþùÖïÕ$"À&ï)~°^j@ƌãfÊã1^p;jÔVÓ^œ›7" Òs€è³/k4kp²è°õɉ.`d°§@âÊàéFJ‰ªf*NŠù²]˜4Y©#.‹·.`¡@{º"…-´zGK_(•Â/º¬èàgžÀyTUÔ÷´F›øJ²]÷w×ìTêÀWÓG™x|ÄwËN1" Lb‰G-pŠÿ5¼•g
êË°é(©Yj¤Ã.Ðaê
x™"³Vu9À;:œP]‰JuëIå%Iµ®¾L\g+ï
UX¬Ì¼öj,ÇxP]}ñdRU"Ⅶ\ízš,uë©àŠnk¿‰*¦Uí]Ñd6†?8*ì
*õ¶v¦€W±ˆ©ú&Hòdê.¡Jªì¶–%K*ð7Èœj؆S
qªaN5lÆ©†­8ÕrIª9Õ°§6ãTËúQË©–:ª9Õ°	§ZÖÓZN5léNV±wªå®Ôrªe²ÔqªeE¯çTÃvœj™0õœj §zh€=²|u"n5®´
÷žÐ†:žÊå<ºþ²"BÑBóæË͞áãŸ*ð
endstream
endobj
34 0 obj
<</BitsPerComponent 8/ColorSpace 35 0 R/Filter[/ASCII85Decode/FlateDecode]/Height 32/Length 209/Width 40>>stream
8;XF2>n2B=#_RE]rg2kTFreV"1FJF+fL5HYZ$b@q2UtM#%YnTr'Qp;R$)ZU.*s6Q@
LEbbs^&o=-G@o[j`KFia"F/4VQ1=QC1LG[a?!BraYQ!O6s5cB*5)WZ>,-(>bnJtTB
Ufe_QJ'A>cqe,]8DC2%=>OcUe".'qEn@k9B+*C@"nlaO3dsEt&;6cWS5>Sf7=i4$X
0#msHD.M#~>
endstream
endobj
35 0 obj
[/Indexed/DeviceRGB 255 36 0 R]
endobj
36 0 obj
<</Filter[/ASCII85Decode/FlateDecode]/Length 428>>stream
8;X]O>EqN@%''O_@%e@?J;%+8(9e>X=MR6S?i^YgA3=].HDXF.R$lIL@"pJ+EP(%0
b]6ajmNZn*!='OQZeQ^Y*,=]?C.B+\Ulg9dhD*"iC[;*=3`oP1[!S^)?1)IZ4dup`
E1r!/,*0[*9.aFIR2&b-C#s<Xl5FH@[<=!#6V)uDBXnIr.F>oRZ7Dl%MLY\.?d>Mn
6%Q2oYfNRF$$+ON<+]RUJmC0I<jlL.oXisZ;SYU[/7#<&37rclQKqeJe#,UF7Rgb1
VNWFKf>nDZ4OTs0S!saG>GGKUlQ*Q?45:CI&4J'_2j<etJICj7e7nPMb=O6S7UOH<
PO7r\I.Hu&e0d&E<.')fERr/l+*W,)q^D*ai5<uuLX.7g/>$XKrcYp0n+Xl_nU*O(
l[$6Nn+Z_Nq0]s7hs]`XX1nZ8&94a\~>
endstream
endobj
29 0 obj
<</Intent 37 0 R/Name(Layer 1)/Type/OCG/Usage 38 0 R>>
endobj
37 0 obj
[/View/Design]
endobj
38 0 obj
<</CreatorInfo<</Creator(Adobe Illustrator 16.0)/Subtype/Artwork>>>>
endobj
33 0 obj
<</AIS false/BM/Normal/CA 1.0/OP false/OPM 1/SA true/SMask/None/Type/ExtGState/ca 1.0/op false>>
endobj
32 0 obj
<</LastModified(D:20180321112203-02'00')/Private 39 0 R>>
endobj
39 0 obj
<</AIMetaData 40 0 R/AIPDFPrivateData1 41 0 R/AIPDFPrivateData2 42 0 R/AIPDFPrivateData3 43 0 R/AIPDFPrivateData4 44 0 R/ContainerVersion 11/CreatorVersion 16/NumBlock 4/RoundtripVersion 16>>
endobj
40 0 obj
<</Length 999>>stream
%!PS-Adobe-3.0 
%%Creator: Adobe Illustrator(R) 16.0
%%AI8_CreatorVersion: 16.0.0
%%For: (ARTUR) ()
%%Title: (SNOW_LDA2.pdf)
%%CreationDate: 3/21/2018 11:22 AM
%%Canvassize: 16383
%%BoundingBox: 96 237 517 553
%%HiResBoundingBox: 96 237.75 516.001 552.751
%%DocumentProcessColors: Cyan Magenta Yellow Black
%AI5_FileFormat 12.0
%AI12_BuildNumber: 682
%AI3_ColorUsage: Color
%AI7_ImageSettings: 0
%%RGBProcessColor: 0 0 0 ([Registration])
%AI3_Cropmarks: 150.75 272.25 476.251 530.168
%AI3_TemplateBox: 305.5 396.5 305.5 396.5
%AI3_TileBox: -95.3994 115.6094 722.4004 686.8091
%AI3_DocumentPreview: None
%AI5_ArtSize: 14400 14400
%AI5_RulerUnits: 2
%AI9_ColorModel: 1
%AI5_ArtFlags: 0 0 0 1 0 0 1 0 0
%AI5_TargetResolution: 800
%AI5_NumLayers: 1
%AI9_OpenToView: -3.5 542 2 1235 603 26 0 0 82 116 0 0 0 1 1 0 1 1 0 1
%AI5_OpenViewLayers: 7
%%PageOrigin:0 0
%AI7_GridSettings: 72 8 72 8 1 0 0.8 0.8 0.8 0.9 0.9 0.9
%AI9_Flatten: 1
%AI12_CMSettings: 00.MS
%%EndComments

endstream
endobj
41 0 obj
<</Length 5331>>stream
%%BoundingBox: 96 237 517 553
%%HiResBoundingBox: 96 237.75 516.001 552.751
%AI7_Thumbnail: 128 96 8
%%BeginData: 5187 Hex Bytes
%0000330000660000990000CC0033000033330033660033990033CC0033FF
%0066000066330066660066990066CC0066FF009900009933009966009999
%0099CC0099FF00CC0000CC3300CC6600CC9900CCCC00CCFF00FF3300FF66
%00FF9900FFCC3300003300333300663300993300CC3300FF333300333333
%3333663333993333CC3333FF3366003366333366663366993366CC3366FF
%3399003399333399663399993399CC3399FF33CC0033CC3333CC6633CC99
%33CCCC33CCFF33FF0033FF3333FF6633FF9933FFCC33FFFF660000660033
%6600666600996600CC6600FF6633006633336633666633996633CC6633FF
%6666006666336666666666996666CC6666FF669900669933669966669999
%6699CC6699FF66CC0066CC3366CC6666CC9966CCCC66CCFF66FF0066FF33
%66FF6666FF9966FFCC66FFFF9900009900339900669900999900CC9900FF
%9933009933339933669933999933CC9933FF996600996633996666996699
%9966CC9966FF9999009999339999669999999999CC9999FF99CC0099CC33
%99CC6699CC9999CCCC99CCFF99FF0099FF3399FF6699FF9999FFCC99FFFF
%CC0000CC0033CC0066CC0099CC00CCCC00FFCC3300CC3333CC3366CC3399
%CC33CCCC33FFCC6600CC6633CC6666CC6699CC66CCCC66FFCC9900CC9933
%CC9966CC9999CC99CCCC99FFCCCC00CCCC33CCCC66CCCC99CCCCCCCCCCFF
%CCFF00CCFF33CCFF66CCFF99CCFFCCCCFFFFFF0033FF0066FF0099FF00CC
%FF3300FF3333FF3366FF3399FF33CCFF33FFFF6600FF6633FF6666FF6699
%FF66CCFF66FFFF9900FF9933FF9966FF9999FF99CCFF99FFFFCC00FFCC33
%FFCC66FFCC99FFCCCCFFCCFFFFFF33FFFF66FFFF99FFFFCC110000001100
%000011111111220000002200000022222222440000004400000044444444
%550000005500000055555555770000007700000077777777880000008800
%000088888888AA000000AA000000AAAAAAAABB000000BB000000BBBBBBBB
%DD000000DD000000DDDDDDDDEE000000EE000000EEEEEEEE0000000000FF
%00FF0000FFFFFF0000FF00FFFFFF00FFFFFF
%524C45FDFCFFFDFCFFFDFCFFFD7FFFA8FD1CFFFD05A8FFA8A8A8FFFD0BA8
%FFFD0FA8FFFD07A8FFA8A8A8FFA8A8A8FFA8A8A8FFFD07A8FFA8A8A8FFFD
%0FA8FFFD07A8FFA8A8A8FFA8A8A8FD7EFFA8FD1CFFA8FD62FFA8A8FD7EFF
%A8FD1CFFA8FD21FFA8FD0FFFA8FD0FFFA8FD0FFFA8FD11FFA8FD7EFFA8FD
%1CFFA8FD15FFBCB5CAFD7DFFB5FCC3FD18FFBCB5CAFD2FFFA8FD1CFFA8FF
%FFFFA8FFFFFFA8FFFFFFA8FFFFFFA8FFFFFFA8FFC3C3A8FFA8FFA8FFA8FF
%A8FFA8FFA8FFFFFFA8FFFFFFA8FFFFFFA8B5FCC3AFFFFFFFA8FFFFFFA8FF
%FFFFA8FFA8FFA8FFFFFFA8FFA8FFA8FFA8FFA8FFA8FFA8FFFFFFA8FFFFFF
%A8FFFFFFA8FFFFA8A8FD4CFFCAC3CAFD2FFFA8FD1CFFA8FD62FFA8A8FD7E
%FFA8FD1CFFA8FD21FFA8FD0FFFA8FD0FFFA8FD0FFFA8FD11FFA8FD4FFFBC
%FCCAFD2CFFA8FD1CFFA8FD31FFAFFFFCFCC3FD0BFFA8FD21FFA8FD4FFFCA
%C3FD2DFFA8FD1CFFA8FFFFFFA8FFFFFFA8FD07FFA8FFFFFFA8FFFFFFA8FF
%FFFFA8FD07FFA8FD07FFA8FD05FFA8FFAFFFFFFFA8FD09FFA8FFA8FFFFFF
%A8FFFFFFA8FFFFFFA8FD0BFFA8FFFFFFA8FFFFA8A8FD7EFFA8FD1CFFA8FD
%62FFA8A8FD7EFFA8FD1CFFA8FD21FFA8FFFFFFC3C3CAFD09FFA1CAFD0EFF
%A8FD0FFFA8FD10FFA8A8FD41FFB5FCC3FD08FFC3FCB5FD2FFFA8FD1CFFA8
%FD25FFC3BCCAFD08FFCAFCBCFD0EFFA8FD21FFA8FD7EFFA8FD1CFFA8FFFF
%FFA8FFFFFFA8FD07FFA8FFFFFFA8FFFFFFA8FFFFFFA8FD07FFA8FD07FFA8
%FFFFFFCAFFAFFFA8FFCAB593FD09FFA8FFA8FFFFFFA8FFFFFFA8FFFFFFA8
%FD0BFFA8FFFFFFA8FFFFA8A8FD45FFBCFCCAFD0AFFFCFCFD2AFFA8FD1CFF
%A8FD29FFB5FCC3FD0AFFC3C3FD2AFFA8A8FD46FFCAFD37FFA8FD1CFFA8FD
%21FFA8FD07FFCACACAFD05FFA8FD0FFFA8FD0FFFA8FD11FFA8FD45FFC3FC
%C3FD36FFA8FD1CFFA8FD29FFC3FCC3FD05FFA8FD0FFFA8FD21FFA8FD7EFF
%A8FD1CFFA8FD3EFFC3FCC3FD21FFA8A8FD5AFFBCFCC3FD21FFA8FD1CFFA8
%FD1DFFC3FCBCFD1EFFCAC3FD22FFA8A8FD39FFC3FCC3FD42FFA8FD1CFFA8
%FD1DFFCAFD13FFA8FD05FFCACACAFD07FFA8FD21FFA8FD27FFCAFCBCFD29
%FFBCFCC3FD28FFA8FD1CFFA8FD0BFFC3FCFCFD23FFA8FD05FFBCFCC3FD07
%FFA8FD21FFA8FD28FFC3CAFD54FFA8FD1CFFA8FD0FFFCAFD52FFA8A8FD7E
%FFA8FD1CFFA8FD62FFA8A8FD7EFFA8FD1CFFA8FD21FFA8FD0FFFA8FD0FFF
%A8FD0FFFA8FD10FFA8A8FD4DFFBCB5FD2FFFA8FD1CFFA8FD2BFFB5B5CAFF
%FFFFFCFCCAFD0DFFA8FFFFA9A9FD1DFFA8FD46FFCAFCFCFD04FFCAC3FD09
%FF7F55A9FD05FFF92BFFFFA9A9FD18FFA8FD1CFFA8FD2BFFCAC3FCBCFD0D
%FF2BF9A9FD04FFA92B2BFFA9F92BFD18FFA8A8FD48FFC3FCB5FD0DFFA9A9
%FD0AFF2B7FFD18FFA8FD1CFFA8FD2DFFC3CAFD33FFA8A8FD53FF7FF9A9FD
%28FFA8FD1CFFA8FD21FFA8FD0FFFAFFD05FF55F97FFD07FFA8FD0FFFA8FD
%11FFA8FD4CFFCAC3CAFD2FFFA8FD1CFFA8FD19FFA8FFFFFFA8FFFFFFA8FD
%0BFFA8FFFFBCFCBCFD0EFFA8FD07FFA8FFFFFFA8FFFFFFA8FD0BFFA8FD04
%FFA8A8FD4CFFC3FCC3FD08FFA9A9FD25FFA8FD1CFFA8FD3AFFA9F92BFD25
%FFA8A8FD56FFA95555FD25FFA8FD1CFFA8FD62FFA8A8FD7EFFA8FD1CFFA8
%FD21FFA8FD0FFFA8FD0FFFA8FD0FFFCFFD11FFA8FD5BFF2B2BFD21FFA8FD
%1CFFA8FD19FFA8FFFFFFA8FFFFFFA8FD0BFFA8FFFFFFA8FD0DFFF92BA8FF
%A9FD05FFA8FFFFFFA8FFFFFF7FF955FD09FFA8FD04FFA8A8FD55FF2B2BFF
%FFFFA9F9F9FFA9F92BFD0CFFA9F97FFD0EFFA8FD1CFFA8FD0FFFA8FD21FF
%7F7FFD06FFF92BA9FFFFFF7FA9FFA9F955FD0CFF2BF97FFD0EFFA8A8FD4D
%FFF9F9FD16FFA9F955FD05FF79F9F9A9FD07FFF92BFD04FFA8FD1CFFA8FD
%31FF7FA9FD16FF7FF955FD05FFB46A2AFD07FFA92B2BFD04FFA8A8FD65FF
%2B2BFD06FFBCB4CFFD0EFFA8FD1CFFA8FD21FFA8FD0FFFA8FD0FFFA8FD07
%FFF92BFD06FFA8FD10FFA8A8FD65FF55F9A9FD16FFA8FD1CFFA8FD19FFA8
%FFFFFFA8FFFFFFA8FD0BFFA8FFFFFFA8FD09FFA9FD05FFA8FD07FF552BA9
%FFA8FFFFFFA8FD0BFFA8FD04FFA8A8FD56FF55F97FFD25FFA8FD1CFFA8FD
%0FFFA8FD21FFA8FD05FF7F2B7FF9F9A9FD04FFA8FD20FFA8A8FD53FF55F9
%7F7FA9FD26FFA8FD1CFFA8FD37FFA9A9FD29FFA8A8FD7EFFA8FD1CFFA8FD
%31FFA8FD0FFFA8FD21FFA8FD1BFFA8A8FD61FFA8FD1CFFA8A8A8FFA8A8A8
%FFA8A8A8FFA8A8A8FFA8A8A8FFA8A8A8FFA8A8A8FFA8A8A8FFA8A8A8FFA8
%A8A8FFA8A8A8FFA8A8A8FFA8A8A8FFA8A8A8FFA8A8A8FFA8A8A8FFA8A8A8
%FFA8A8A8FFA8A8A8FFA8A8A8FFA8A8A8FFA8A8A8FFA8A8A8FFA8A8A8FFFD
%04A8FDFCFFFDFCFFFDFCFFFDFCFFFDFCFFFD1FFFFF
%%EndData

endstream
endobj
42 0 obj
<</Filter[/FlateDecode]/Length 15892>>stream
H‰ÜWYoÛ:žçý:HÆÑbÉrúä$Më™,†ævP-1š(ÊIúëçZ½+·½w<Ad‰çãÙòÍߣÃ^$&äÐmYèõ«7oN%ÁJÈcd–QŸ±4QR/ß"ÛoYÕëãyKdB?6´Œz®÷ô†7ŸaËÁ[½tC#°8ººþm|qÖsZqt÷¶ΰ€{äØGŽeȶõ.
ó9Núƒh1nàêÅ'òˆòé‰x:F]9ny6ü{†ü‰I²Óêx]- |Ú~&ÂtF¸H'$9LÈä>cŽ.ñ(ý‡0&Ñ	Ãáìéõ½ñ9e̝a…lÇXßëÛÎø$¥,ºJgžðǬ»cÃõs쀳~7ëqK#¢¨
B‡OêºÀªù;ø:$SjBNûö¶à,E<Ãòv۞¥mt:NËñP»ãØêZ-Ûrø
™ÅnüâZ^ËCn××Ï꽀'…vØõZn·Û†Èx-߂—Žã´Ú–ÕýV`uí|KåK2§äñ]	Nr‡õ¤eqlÃÖ왓†)#ò3§
ŒÈ<ÖÍ<v)"Â`GÅâœaã(ógWÏqƒå"(ˆ¿`©2É"R *ø™èàÚ¹ë˜ðqkT…B€üh;ȁ€ºò-9¾'À'í—Bí꙳Ö|4—'GÇq¡½–tJùq¡`güQÒ¨ŠwÇAAö0F´'Ú·øÏu˕"¼Príô²–9Vër¤¥~àÑ©˜é $¦V g8¤ӜZ}°HãÜ³0†˜
$åšñëWW-X
ďR¤qŸß‰×¯²>qKBèØ]O¾Ã¾Éjt#q<à»Ä´0ßî`vJ'2*ì5Ÿð{§›ì?#wP–ƒlõŸ&âãróý†e܄ù€aŽ%2"'÷ƒË*îÕZ#¶518Él2˜%[5R#QXÝC##<JJîÙç'òÙb–£çÙD0šÌJ†õ•ò½¡vŠH~Í35ešÜ£!Xåˆ"ª K•íÙ!%x î/óS̝JßÓpÿ5ôRІ½²(4^_'q'T
[ݱOrŠ$úQh~Êz+fôˆUxíe"±¤dG-êðÞQ¢£"*RÅKÌb}B£{ëe<¯!+¾ÞD}î
݌¦Ç»zf¦ÎÑ¿¹xäækpn<ºÂ3'ÞyDáBJº…®õcªv>d¿<ë¯ÁÛwX{D¶….Ñ×oŠ^q˜A¿DÀ,ë»ï_¿BGÐùõ˲ø¯°ŽS¦¾íÖ¡šðÀë-
U–šµüN×\ób9pF…álÙ~»Ð¹÷"ìͯB$j>Ýœfp ™ƒIs½—–Æ_~hÏ-Ÿ8!üŸTڔ2_–#Àt!0«&gß™'¶•³Ñ£Yý­XfË«›$äJgZ¸¦@F¼:oô'
µ{°|ξ\^\Á¹uù=:xš1€C(~I'©"0‰ßpOJü§²ùERj¸ð.@'ðå £>¸ª$ë‡zÖmȐþɓñËä=ç$ðé"vŽYZ'5!ÙäPÙ9.×&Yüü¿wtQÒÄKL"$jä¦ún/œÀL…í&FBÎÀÍåÊXÓÀÐ:üW&ÅÏ;ÅÞî"f® xÂH£Êhéÿy"覦‰³?°-셕/k}ÇóæVjì‹2ýMÑãë󖞡P‡Í3õϨPhßôùk•rr÷¸ÿã}Ê$a4üë´ñ¶cµ,¼2$˜m±ú'Fê¾QØsä^´o×öYwOèô¾Qƒ)¡{aŸãvàþ¸Ó¼çF–=ï‰Q]§AOÍОùw"Ä6{&BÁ9ê'Ü©kIá:ÛȼÕM{s"0=r$R''òh?Î0âöBQ8'CÖ/P¦ûÓÊü#a:#¼Y÷«¡Í'•Ë?•"îI'{PZs²&ÛVª.°\_÷®Àò:­Àu²šʕÑü`˜2"2»vF"˜áçK,
+zRM–Ò÷ÒϜ† yaMíBYN'AoXÀŽßr<9~kZ	»ÃLL£H¨¶Á'¥gi3<×jÙ~Ð|¿½ÜúIaĹÃ)SWëò À×V~ÉXôú]ã˜H"ÐYÊ°¶"µ'g…'	¹ÔÃ4@I̓Cš…Ïh*iü~ºxNÛ	6rCšTÙµ;•¤Ìå`I¢ê{žëm†Úuvbë:ìW:ؾ¸%ô,¯‹SÌç8UàØ6H'9'è†<)ô!¢
O(£ªåÁ×KÑt††$,Õü¶šÑ†U!ÁU$Ñ9"[±72ª§½g‰¯º$É=âDI˜$©‰+NNÖ–ëTũڵɶJ¬*xù4ÅS'"Nã¢E,··þ1Ž¢åŸáäaÙ¯I,Ô23ZŒ¼N'ØQL[EÍçKTYõ¶^õR%J#ÉjyUED\"œ2•¢´g–'£°"–"GÂ"ڶ߂ãw­ó>ôúç)c…ën‰LÀ;@-ÂâtüN®ýˆ11
÷#Ôèx¨¦kÉlmž¬¯µØa™ôU"­^Ç8¬'¹ímŸãôø"'p}ÆYAU¹¥ä¼	cBa»ë  Ý^4ËûG
—mºÌ6{÷¶3²ÃõPÈKo³Æ=žT5g·€µs°m/è´7È?gBÈzŽlK(®åÉNl"<1ÀÅ<q|ÇÞ¤°¶®®¯t{v)­· ›(k׺î°ëîZoÙu7aO	c§p..îF®Y&ÎfU?	hY'ª_OëÝÈBw儀®Å('HÁjM"å=¢ŽökhÌEÐ|qt6àfÍíhIr\ŒJ1'2†ö¨';BFcÔ³˜''ÔS¨ár‹UMõ=Ò4ûÃ9èó}'Y­cXèÐ+Æà–º‡ƒÖ&n1§É=tŸz÷Úp¾
\»³›—ŽÞ" :òe½µ››-·4¡ÙiBw°…¾×é6è{§/è߸uV,NÌít‹³Ø°jÄe­';]¯¡'ué¾Ð'Õ…£Ï#ò4"¡àÑ7S™ìdeKÄ6í+MúÙ@—Œ~wœK«aîtì†aÖLÖFù½Þ
'hÍ1]	µH/&ÂTsqC꟭;c®Ù|°zÀ>'ö é$U$9ú.&­â÷¢ér"–±p¨d«±\FIò_Ϋ´-m¦ÿ•ñuŒ'Š¨,‹ÅjÅJŸº´C2HHÒL¢µ¿þ="0löC{©¹Ï2g½L5J˜ևð#–¡îìàtî"?Ó¬qEh6ïjšæªæ'=
Òã3 Ž.ŒQOWÄ¢œ1âqA©ö³¹>+'ÇãÍñl*Ÿ&²¡(ÂÈ-CñÇâgؚÒ|Ô»ÃêJ€'·Ù¯~ôó÷"Q°£Ù÷¯ˆ•q£Ád©­	²§ÒÍKP)õÉäæúÂB!SžÁgMÏî—)gW/9B¼‰JºiZs\R*4wÀ'l‡ûB92É}Ue{,ޒpœðT©«OA7	̪ŒPÛð¯Áýƒ½x?=°ÅùpP>Œ÷փ‡ê6ÜLF£7$Z0U­ä¬05\²#ÛJZa<j²D5ã"<)NP·Œ[)fÃ`£)ÃU&Të˜!å¤	8*.§ét'†¢®œxÑC•z³,[»0±pbVß®YëÖ0(›š†ô 
h5ŒvÉíµr$ܒ8/€BáðXŽD*@Ã'†õ×o'˜iP5mÈ{†ÇBr1ÎA/<׏†Q	k$Ж
|Iy)•LMzK]HÒW(á2È6§S_	)Ó°™!s`ÒÜ
GtK.qD3µß´Œ›ÅÅ{3k–,Bжj/úK(ïÇ.rØì,]T	[<
$YÁԎÅ0Z¥ÕIñӓœJéÏ®¡Ö[4)¥a2­¢h›W˜ßFXçIô"`ޓ¨ÎRt[µ"‰èLK1ôÄqÈpÔ]º•-
Ï}!I\ #•'Þ¤¤SA'cÌn d"Ü	˜0M©!"½¤§hÓJL=ùH'.'-†"¶GŽþ-â©o	V‹ÚLa"ᾐï^ÌZ¹
Jû1ÐqÔœ¯L›üIª·:ۘ&f…˜l붊5ÓÐ؏B¦"4q\MJ¿‹àn¹$²êÌÐMŸ"äSȉ%[4Ã*qaŠ£KI5だjlÂÕMÊþp…°®~
ÑN,,õސf<ÓÊ'êزý¯®> —rÊå7.È3Æ(
 vºÁ¿dØ, Ö'foӄsHÞ'äÊ·z¥ºf|µ|<U‰[%mÃÐ\à>'kיßC×ê¢]K!Òm9/q€-£V[Xfôa]F—"N¸êZ9¾T68jYžÔ-ôߪTØV	]ÞoÌËbmƒC¤( ÈHÕ Œ²'äFò+Ádw^Êc£/¡^
b^eàLÔ
Î)Oc†ãÌÔÈ0>Ã4{å،'¡;´h"Ýìv1ƒIícn0µ‰µs…`X¨Ø¥%ì•8š9X^'²G‹¡ÓÂåéÌ/œ°0.&b(cÈæ—c8íGMÐœáÜR埛ˎ­`&Æë'u1ÅZ²1"èZìÎËضaÚ^,ÂE{aŒÐ•÷‰­VÛãÓÌÃê_¶Ãf
ühª£/†}C$ÒarÎ+¡§iŽK!&"Q°£Ù)H²F\­œ?Q$Þø³ã'uW•tŸùøsVr0Ýo'Îl¤cU£":Œº‹Æ«N1«­Ïª.óS+«ÜÊ*—£HRŒtoGIkdt²š&ÛYKÞåwˆ}u0×ò~ªÉ[؁\‰$fÂÂoÿÓ°Ø;C~WD™èûº$õžx2Ñw"óÒÐ
ib3ÔJbP™pB\*™ìFG'ɬKRˆu	§àí›Låp•/úR·–:c"C'vÃúWŠƒ°N+x5¬i?圍¼ùg"·†ùOrmÃæHlä¹äËà°Y¸o`$&¾Ä|	ßZX§&¶ˆ.ùµùþãaI'|÷ö7È9Ž–<œ³;w‹ª™÷z$i‹zÉ.R.ÁÎ1—¿1`-3€4ic¾êiˆpsÙkà¦c§ù"*g™‰È½"½-sSšÝ¨¬Ù®
M•Rv_Ùk7÷Féé¬åeÁ'£Âc/˜PÒDºžŸ'-É2FØîã7ð7ƒ›"¡¶ª»±y˜rFˆs¥—QØK(¸WÇ<\ïW˜'"ÐÛ¿š‡ÔÊ*ó¿'ƒª¢×Ý¿©áëø]û#k&…."ÂZÌræ«Ìr›iûÅ£Ò£H*Tné<cï×Çlb— ª<͏ŸÁm™ŸôIqƒd³e"…Fºzá8fPë/¹lôÔ[¼°12?Û€éàÐJ%¼m´yþvIA°Y=!Hön[å…¢×	ÑÅ/¬'±Žø{Õ"ýyqÑȆäÌ ¾ôº*áÿ°²7ÃA&"'AL¼ô»¦=uc¬êH
*"0ˆêðZdL…Dj30F†o6¦	µì
yêHæ^O‡y£Žõ…ϚuÀ;CY˜W)rô©í%de'¥šp`c]ÆV
-­¸Š
ÉMlŠí8$£;•¼f(Åà´Í\[^ãEÙk~&¯»öt%…ý¸J¡†\
,R08ByøæQ—Npú'o[õÏÝÖ Óë싄%ÑýZ9½Úº/4†Ç¹#ü½x±·uµÝnZç³I}¬¯]t׊ù\GÅݨ~ûtV]¯7¿Ÿ\VNëý‡ÜeÓr¤Z÷¬|y°YªTÖww©ø,Ž‹»Í£'ác³Q4i"~.æQÍòQv{üék¿Ù¨AG=>'DAȍWlõåÿÀ`MìnÖk?Îmñù±]ù±]l͌>mõö¤pR]wºbecØ~ÖrC0#*»£HmµC¥v÷õþ¡uÛîâ­ò¸úc³1í>6ëT˜Äâ¦Ó͟Ë
˜qãÕýÛCT‡µ¶ÖԾוöÄîLj?J¡ˆüÚ¥Rÿw³qšzŠÀiÚy?ðÓÖo±'÷ÖÚÛÏ­Áöºî9ñ˘9|Τ3iÿk¾3©ü<j´6÷¶
í/Å_…f'÷­Û!ÎǓ»‹õɑ$á)ûI-œ)ý‰gº´»ƒk–ºñ«®>]Èmmó4·mœV°õ›=àCóèb²fªGwÍ–.åf…ãË£ÚìáX­Õv¨²×²¤^©0­—•'xAï rµ©
÷våºÚÙÁäÒåq~»HÚZízæ½á¿þf³Ók¬ϊ‡û"å¦w_]?©uŒ§BãN¾¯—G돮Þ}žtRý¸ÎÒr_V¿ê,T'íé‡êö¼@ïäþnéqýRÜÁ­îZá‡ÅÌTه'W‹3»£ÿõ*î/…"ncþScxöÙÃwŠg¿<måÿÊ=¨àﻅ""³bY<Ï
Gòó—'7›Ç ïª½ï›Tû"páqáB)|ÃP¤âþm­-þtÃ
sñ´RýQ}–Z·âsATv>ÿ>Ã8·Ñþ?÷Õµž<'DŸ"E'0HdP#rNLÈ™÷ß	ŒgþÙÙ«½ñ'ÓÕNª®¢'Í*[qwšBY+²^_ùãWÒfÄX·1€öèYOQ–ëeU^µGÒrEGRúÖm¨'NPÃô˜aj³½e0Q?n5¡\ 4UöÏ4ŒÎ
k\—C¸È´¾8¤4øæSË›ÐÈ_®?ƒ{׆Ä-"㦪*¨,]€¥7sÑ1—'IuÀ¿#pcN•Gˆ`@ܳÃç|='kOî-˜>™ÅùŠp'ÑءʲÂ(O!ÞpCj¬út-,\£õ»†öäúZcçªÏsðKº¶V…°jñÔAwšM]™A¢ò º¶œÓ/å̤¦ÍšÀô¢íç<Tr›Öƒò·¬
NØWia×sMf"FqÍ&ÍÊb¡»~å/µÉe»ŒŠG‰'Ñl¬ø">—Šê¯lRªïEéì8ÌX¡¸¦ºªÈqF¤Cåê=a*×
"«rd| ÄÕe¶7»Ö^h,:. CÜ"à¾U=!¦/Ôô…\ûòˆt °0[§_Ö½9ø»_à–¨´:¹[G´¯Æ»ÊØïÇò$¶hM÷ôü(çjþ&±Ú"8Ôݬwš±öy'×¾ÃR岔ÏÖê{5âÛx[l­›"'WÅ÷ql[/ÏÓ)$´ïÂÀÁyý‡@bH}žuп§Î¸H]7}¡>ÎKæ)+Œy.'…È¸úAÁ#R½ëH¨_1ë	Þ~Ùò§i҃Sf/ÔH—Ë"¥ÃhßN2éó¤æÛ*àÏL$5j&à¯|÷ƒ_4ø훷ÿF"ºÍØE¿Í›šÏn7WàËÏVð%óúÍV"µT —©¯•ŒELáƒiæî "²+Bf¶ò³›û÷ùõL6ÝÁ>Aïà2ƒ#E*¡[~±Ž3µ¡¸xý¥»ÓÏVœ‰Ї£égl×ó—2¤šð§/ØÑDö}Cþ$Wµ€!íyK7-CÁšyÌÖëüþÓd<eÂ2udoxWMù~úÕ"XÎú"ÑšþéÄoÑüIZPøë¦Ò<}øråæzü7zŽ'=.‹/?ñBÈÌ+¼p¸Œ"¶¨¡ðK\AlQ›Z =.™ï:ݱU+¸Ÿ~°
õa«4®+e©ÅðA•X€ñªdÌʄ×`Ø©Šl­ÌÜ@
÷ߒ¡ÞÁÁ٘vϾu	×£!ýWdDi1Æ ¡š†Öýtùö…B'àX½ƒÇ™-m§òÞyìzÔþ~°Â¼žFA»IÕA"á³FÎ'ÉÄm¹À<#¯ù¶³iHËáˆW¦ë£¿m¶#~©ü¾îØg'@­;p[{Üx«²ògðLXùô¬Gïa#|Ëëc¥ÅµÖ"5í(ÚCGs¡¶"Ë|}xšÀávÃo©G3´Z$KäfąÆêþù4òæïƒEµuP¦ÁFD¤ƒÑmµ¤Ä‰!Ï	%g\h€Ê_Ys:$ʶíÎ>Y€ýõ"Ý.؍º×ñØöCA'®…ö'bm @Çàfùxïß,/°¹ ê_./°¹ÜÆÁ;QC0¸	ž]«3­j 4¤áÚÚ`›ð)gæ¡é^›cS'/¢	ׂÊRõ·x0§¥k|Û¸rYi/°àŸˆU¾OˆU÷׍Êd>K1/ ²¯*ˆýiZ˟+æÛB.<3Â.Ç´6…†Pnj€ö L1G-O~Û90¤iš&îu7´ÑG»0c­?]—åìÚ=uVÓ7¿™'¯à%{x›°l +=ê-ü²Ãp^³Ùd…ú†€ëƑšÖ2å(ßt°æ:Û æ¯u6±þïõí­ÒbàHG£¾Â à0ì⺋JEÝ%	÷†¡¸Ž~8¬ƒ;çÉäl»!aªò¶
®\ E•Sá»F~NUÙ]ayFÝì6ùtEú	fZȋÕ
_‰ú»Û'éêµëª¥zK•ý³ÛA{õn¼÷Ìú:©…Cx"=—ç§'Ó·ò|²þ¿6
Ìܙ©ò§Ó¢KÛd!EfRc¸J¤ÎJŸ6å僘cW'¤'ͳã!ý¡À¦´Ðý ;†—Þ֔ zËçTÂŒÖÕPp¶ÏUMUG~ÇÆúÎs"áŽoWžä"P_'א]!ºÛzu¹@h08
—lšÎ…äü‰›Lûɇ'Æ¢÷J~Ðöge¥z!Óþ¶'ßeÌOþ ŒmžÀ2Ûâ^—–ç%
»€ꃡB9JO*Ùõ\"l—í2:ˆZ‰'Ñl¬ø¬·êù­Œß©¬¤mH'J8J°ø»•‹ u©Îå‡VšÉ³-¼QÐ÷&ëÞ)K9'~œB{G:¦r­ z³ wñä|왛På*q®Q@i}‡f`Û,5_Êhèî÷
‡¾û¶¸³ô`Úå`°Ÿð
2"I¤·|œlPÿîÓ½ñm>áPL»x¨?¾çX"áޕ¹2,OF`bIÁÞ£û•i€1[­°ÀóiÿÝÉs™¦GþÜ.ûb¼Õ	U¢bµF@…uãÎ~1⚚ì~`>"òg¿@À	¤†D@¯æê¯ÜO4<®º:rzº² 7	WPÎûü>4òX]†{
˜Á¾¥tW}ñÂj<«µ³ hÝþÞÁ|Fâo¹.—»éH³á /.…b¼=œyäg?˙:îO.t:Y\ézré­Á¬T¹›#^÷ 3©¯}ðWR-')MSå''Ô|è_KÆB9'KFj©÷=
´É8%ÔãêWv{!¼Pnuo6?¸ä<ƒ·¥¸ÀãM†îd¥'ÔÊ<"v&ùf6}rôÁH}¬LóGÛØhª"Ãáö˜I;GþE P5šþP9NÞâրl&rètÈz}¼—–o®8àw¬,ìҟûWDB¹Ü+臨¨G(¡œT4>%ìc¹éçãO!ö
;4/0_³'¬³ãˆÒ›_<O²«"·faWØ/Êí'2÷)
ý;°Üne>mTIÐï¯X®¥!0l
͓#Y¯žá#»†éï(¯®&eµ%ú~ªîFÇPQQÉ¢ŽÅ8f1gÔªûtûí	¿ÑSç¼L1ìm/:­^­ØdëÎdU{2"åbÁ÷ú
çY²u-;"ñdùàeÛ'oLf,½7úœì'^ÀHa·ÇÌÔRyþO}½è¿g+Lf]ØxSь'æÍ¡hݳEkJG®$ð*ÔÈÒÁÖ§ÚÙb<EåÎb ¢ûÙxq¹²(wø£QŸòVྫŽƒ¥o\ø•ÀæáS
œëà|ÒÜÂ=!­QJgQ鏢o$KŒÛþUƒŠløM)ù]4ê'Œ³UÛP‰Hü
§Å©fÀ>ˆO7–VÌ»ƒÌ—ŒåYÃÖ;‰ÓxQ·1˜£3·elMY˜¦‰GÝö¤¢Ðb?é%ۛËŽ¬æb&õ5Ý£¨6¥·¥q½}¼ÛMÈ®¬Þ@h±ESœ0=´Hœ½Ѽ08áq¹éˆ'h€XÊ,¹Rˆ'8­ž^±Ljo³6åMÁ"´?úÚTªFJ\ğWe"^À˜·ÌOíÉaíåú"¿·Ò8²hÀý"^N.Z-Ȑ‡V™ÛqS׈~ž~gâ
ŸÅ^f«æÀþQË>Uÿ57ïÀcó]Yüí¬m9<œ–U(­.[FDd•ýávÙ·CBºTS¦Å®¹íع¹Io2×ÎYc¨Ë¯£¬ÝÜ4 T*xC•êà'猨£÷Oãî+¨'¿;}Y#Šç×ëý‰¿ÍËJ³Œò'4§Uß_MR—n=œp•éÜ¥Í+…§aZoR'ºÂüD3Œ&ÔR™«žká߃#b ü£,Lø
Lž5%
_±¿!ñ8S
ú·Í,<D6ÏEñtlK£âU£–{š£Ñ•†ƒì'""Ð+hc¢—ÓÅ&§‰‹è¯éu³_ôr:ìWì׋b$Ì*½ã—j¥§Èê0BQRgו-%9Ãn{y¢õª4™æäh_V`ݨ£¨ê5»:þÝqXãÔìȒ‰ò"÷{þJýko"vBT´bÓöüz³£ŸÉvú7d[v e"äJή䧢;1ŸWü2WÁ³â"ظÎç&Žè¿fý¥êZ€æ×*BQ<¶Ñàây»ØeΑcE<]îؐTwåy6¿ˆôªçw'
H˜"Ó=cБìˆñ˜ÕÕHJ—+5kœÊÔÐ(äЫÙïŸuä â£'ƒ£3Ç輪vˆÍpso;áɕ®[>%ƒ:«•&Œµšï•xê½.tp%'ñbÿ.
¤¸®5óÀpĉh3¾Ö Î¯ý!-Óêïàa&v7*ºóםº.¬uÛ>(êŠe`KQp~¹ÚÚL^Ì5«,'yÔyŠ*·£Ú@r1¾sgA¥ž"4VÝIK ¯W" ,ž9	ˆ}©Â4rúa$¦ê×ýr~OøÐó‰r#FÚaºr
𔶣ï*ežMš](æsÝÃezå|ÁjwÑøõ"gN}ôÇ©Yi†®^"}
_žG='g" Ü%í%ÒনKÞ¢êÀCyN¿öè5^Mi¤q
q¡>c+vùÍF?7
³eQÐ,#ä]ôï	ºŒ	$%`L~ÃÆn)¥å—,Ñë7Ͷü˜+å•!ÄuÖB0ˆ+uÒ¢~fëhøQÞ/Û¨úƒlh;¥Þ—tÆ»O,å~Šû‰ë›uÆü(7OSYk¾°ÛÑß±Ÿ_"¼µTP
Ù	|àŒPõZ·Î§ÓÉóVi±¥Õ]`Ä6şÊíaÈ߆ğe·'ͼ²AGÓIE׎ˆ¿eåÔÛp'ÆçÏZ<&IÛæ'øƒïMš¸pDù'בÆiG*m:»Ò¤/œx@'¦ëÌLæT¡E֍_ߝËKN«	¨€Éüƒþñðù
€—ìRoš§ÉNQÞö›bwÖÅïè4
1B¬µ³c—ëâMŠj¸Ä`S»È«‰CJ—f"®gw[	yè(\ezّùÞ{96‹Y¢í?q|'•"Lð"@Ô)G¤6HM/Ëøô­trd"hì'Gr×4ÛóÔ&Û±~åêìÄÿRð¶ŸøpqÙPø#·}"ö§Ån{ü‡§¡ûÃw9w§Êd¼3ô‰~}‡ê6ëK[]܍ϛÉö"~a¾
…úüd¶Øj"ÿžn‡ÿù+ˆ¬¯>âA®*d³tDÛúÄ´ìMEQoº>
âAoÁãD §0ɨqâ~ ÞŸÌƒ'ÖN<lz™•b«$‡Hë§î§ao²BÍ17¡$1ÐY̛Z1˜»ØŽa¾ùÎÓæ=Ç«˜¯Ð1?^ãÁdËeâC"Ý*yðuâŠL—)'§	:gÓfüyí‹ëS\éO€1ŒTrÄùöÅ›S´Â4ò®MÖ%£ÓÆŶÜÒä$—‡<\t{…!ìÿÎ9SJšþ‰ùê½,æ§ý4æªÈ/½"0__`îÅj¹Oü9ç¶:Gú*艇/ép¦#©˜b_>\BúyuĺN1ìL}ŠÜ
t&œ¶)=ø7³ÆuGK¼9ò}4ŒÄ±ntÖt'ÕK\¡'_~5	Vu!ñ¿™Á(='gt ¾é³7•Ád˜¨ä®RݾCíÝþ¼úêÝ:"Dž=þµGµËïPÛzl¿Fe°Ÿ£­Þ*#˜—îªIg*.üä^¡zc'yƒJÙlõv1òª	c"­6.óTé%ꧼ¤í["Q~…ŠËÓ±òÕ&[Ò¥=_¸K¶t<"1Z¯}•µ° P^Éݯ¼ÂBtE-;&êæšZ¨ç&*TæHzNíÑëe"êþ]Pd—<jþר{%0?P©"ž°½C=:Ô|Z"<¶u.<Pæ|´íyùª'oCíר¤»åM¬kÅÿ³^­
‰Qô· ùFÔJKi5ÄwZjš¥Ùj[ši>þÿÎÌ8X}a7æÜç¹çRQ=Åq
ÀÀÖÔV[yê©×—:OÉÔþH(.ÛmzcVO²þÚô­CEU[ç]¦¯þ(Óóª<΋XóxBf¸â78|àni´Ø·ìيD­•O:j?$|=KÅb&*¬4«»y¡¶hÑQ˞Ýy­ÿ÷œŠzó1-1QL5öµâéî&á®öµ££VÃZ±(sTÔvù½l¢ÂÜàÀwõÓö3õZè
Ã4µõ¶'£ð
'Mw˜Ý0Ýí§£µ.ÜGå<U‰Ü_¯Àî>ðí!uæi×òÔÇSáiü¡¡ÂJó4:ïóŒ¯ÁSƒ<öFLÔåTþc¡Ö…g¥vPQ¥']Û=½m«LC]¯Q¯Žú'ÍI‡•"†:ölUIŽK.³Þ%
æPo²Á¯¡Ò»¨Ù59y2Ë>¯£ÎÓaÕ÷:ð¼"T#åûbçŠ[AiTˆ=äÅFt?y
[2Š2‹i¨rPáMTÈÐñMê-0‰è•8ɪ8/N#ÙóÆ¢ÆQO}žl¿T¨Ž@å¤üÍBE¹É´b"»³eV™k¨r§VÃÇ;óìm‰æPzn¬§ÒvÁI™ÏâÔÒÒÎÏ%&‹ýód4O.5e®AEÔߧšäP.o텃IýjW		òýƒ,Ônå$ëôP›TOÑ)€¡¼PêÜý9ësE¸ù[¾eŽ"»Â|KœZ"Í€îº^Žñù &´¯êAÖiJèp_1úé%'À¾Ùqgú‡¬Uº.«âO+B÷_TfÖ"û"ô#h‡/4"ûS¥Àú¼)<xϞX§3á©÷&N-A{<žf¯<ãóÇ´0ì\$X§WÂèt"fœŽÖЛX¸šb¼0Šég©Î8}ñŠyÿ°È:½«-O…´¿K±1—ÞŸOBbVõÓOSÃÏöÅåö4iÓä¡
ÒZA°éKXwoþp±ÒUN;%YPÚ~p—Éʌ~š=B²¹"þµX/<E./·–ÓB4|«/…€Ýr«à¤É/7
Érٕϲ¼)Óüž:‰ý
Qâz-‹¾«ø6P(¶å³>Z@¯"ËøM(ò±¿…B>^€ÏîVúgϾhNB´@{MªWÚ>ÔY}L×Ï?`ÏìíÐ>¨öõÒXl½ñ÷ìK´¢GËP¦‰Q÷Ú#²Íè~º©ãZïQSoaß%·¤£&û=6ª§8‰¨p¬ÀB±o1Ph¾y¯Y¨Ï6¨j4k‰ßï5QכLdc &0ÔóR²÷V»Ø£ªX"=A+jòîÀ˜Àëݳc¢¢šc 'ìtÔd ­QV`,ȉ‰ŠV&*Ü+&&*ôž²QÏ­Šf"Ô)#–»­ƒÔz3¼Žþ§—{Æþ=D6ú«®®L>ÖܽjjïAÞÐ6'Ú©ñ'tÐÄÅ݇0	
zŒoóHj<³®ÙûW"ßyã1ØçF æ0´+kc=G>á·†-°ú—Ð@¨ôﮬñ+)Ÿ=`Jï‰mMG¸1,º†Ûe½µ¬ÈèÊ\Zí4ÁŸ~Ÿþ÷®ÍÞÒ2;¼<¸•§Šrcøl1:§øô__jÒ6'=9›>€:,`1´†>›^û`AƒAeÊBÙÞ,ã†M¼Âk=¤â§~0̲âjß¹<zè6†‡MÎôP›žN[ëŽDÉ!Ðßu§ŽvhÒÍ×V¦–nVZF¦¿›CèîäEäÈx±+â''®'íé\öôšWû+ûú2‹K/hv}	¯¢§ï"úö¡GZDß©Z]wЅ@ý>7ÎñÂY(¶<`¡>¿ÂÿÁõ戌(ÐÕr‡a4ÆB!?ªMf{öù-Ó"Ý@õ衇OåüÔð)]²=­<NoOm3¢8'‹Õšç´ÜXý܋zíÓÓf̟[….Wô0«Í·Œùdúå×ü¢×üP¦›ù½½KțÔ"f†aD'^îjÕOy¬Ò@¶®ã¿›{pCo¦ÛN\¯ £ µˆzÛˆyó*ëÆP\4à‹ôåÂkZ÷á°(€yºl"ÐÑ.D`7è)ȨqQzÚå«ÈaÈÐì¬Â‡n~rI/à!·ØU|>ˆlÒ‹m¦mÂk!6`¸yÓ¢©33ÃzÐð´$¿Ò2?_Û={ÂÆð«·aM*ªšÄ¥¤™a• X­=ñIå:ÉUŸJ.D•ErXu¯4ç¯ìKÐÞ&ÈiÐ,)ÿ®ÐÍ2dKëá6yí¦§™AÃ"t~b«6¼N5Zïˆ"N:¿s›0M»´«´Ü}>`œ
³RçÁm¯¯ÞïÍAðãæk&øð{A#Øíè %ù[K¹å¶¹/b»•ò½!"HålÊf:q{ÿ•ðáo§ué3»&D¢dÏiVõMÀ¥¹ç·Ú³'ƒJÕi@}É
1²ù¯`'Õڏä¼¢ 9hs±ÆiBÃÆ&C'ªu«1-Ù/öÆ8ñ£%Prc¤‡…IÈ­ ‰ý1óEŸYÛÜÆfüіǗDÈ\£€zéE'Y¹téd¶·hV|0VÜ#4–²yÚ|rÇ0	«QfeB‹K¡£Y˜M[¯[*€0v'«ü;T 
'YÙ=Ø{¸hBoŽ¼"z +7¹4^¼rðz+†ó³â/x¸y",ªÓ±3'ÈÿyQ¨9Ì©_̊0ÇÅ˶ÙiñB·À¾¡ÄëÈfÇâ…wzl?Ö°f_Tðfg¬q&B?¤e$q'ñX,ä4Óh¬æüðqËߢb³
b;
Ÿ6¤ú^«~¬@ŒŒ`'ö円tFÄzê[Î%än»Ît'
rRÕ,§N¥ÄIúKpã×´óÓ4ƒÎÓ]þØ%rÊÍhŠ[C~āŒTUv8Á3êð00ؼ±I¹ˆ…ƞ­J!—«'6I!–Ùr¦¹%dvBîø8"þÐg¥}˜‡U—Ùá3É/-¹#úl+'Tɬ¹XEsq?=‰Ê8V%¯ªø\üfßȝlè'å®ôªJDº_¶åžiqø ´¸dzãÆ%_ò›T`­´êÁü€À"Ú¤•sø1d.>ùæ'Ù+]ÊðhozÓ0ü*€ß'g¯-Ý·×ЇÞ÷îàhTT9µ¹@XV²q˜€ìñ‡n{Úå«.ú>p9B»Í¾Ý14lñ'ÓkŸ¹P¸‡9â¢ðQæXK€¸(ò+~Y•Í.Šº0Š[ÇYˆn‹ý`¬AÛ+âPèpíìý5O—m:h´Hl7ú1H4£…lÀmÄföíñ
SGkWZÀ§1¤}4'~)î.7VmjÇn`µI…v¿e\È;/€q"½ÎÙ
åΣô½»«(ì†rCP'vë.b7†€¦›yâÇ,2wþ
€ñ.+Íñ"7tb€¹agsðºžcÛZümÉîkÉX]±"ÁՆdÍ>Ÿ괓­ÇMá`,µ¤¼}ËÀ¥(LÈ}ø››dXHTyœóœ•×?Tl½®É¸Æô<št-·93.¬4w¤n«µo2ŽÉj•»íúñ²…Èœa±Ù8^ÄþÌ[ˆéi\tÌÆÇ6g|(YwÏï^"»ÄÔëp²ïGt»Õ?m8¢ óqìQ#ä|{j.vžÿ¬WiW"9ý-PXì;¢â'Ã.h‹
-âˆíˆÊþÿ'I¥¨$dcùRÖá"o½ïÝû99ZGaçéê¿?'£#ÕµùX"ª9Ò;¶¶£ú'ûw"Ö†î»ÃÐ0´?AZ†t$:œ˜ÐŠ-5
Ņü('GÞ²‰»ÃÛó£"3¾'ÏߖGäG^þ 'Þåålrº¯c£e+ýÏȄÐCµ2>ñɊª‰Æ"Lªä,
æ;Š`GuÒÖ¶žsa`hÈÉûF`M-ª@ÑÒònڀÖ8@ACÛ:úÓ2%>
;H鋖>­˜XXn6!¡Ì—Èuºa†¦ÀoÏ­ÛSÁT0ÿ®Œ¦îâ¡V<"p§¿=E	r—V5C¶VdòÅñ´a­ì2ùèËGŽe½!6)|`ku¯WdMeÐ:¸ÉuÝæ6º#(4hh¹þ­kM0ö¯x=1° ܐȆEÅÔ*+vÈìÞÐõš'ãÞbÑҀ‹j܇Á(?Ÿ_Ý"¿ÚÃAÁx[KgžëçRóª^¼Ž.½¤KÍìI·ð»Ôm~/"àçX)Ÿ‹ü›Ï碵 °ö8ÅÖ^Ž¾è ñ<^I/ø®ú‰.N+FkúÕs"‰ÞþxÑx^vVóù…«IÞ¾_¬+mÀtýàtu§™:	²ÁÜ
ÖI=¼l¤?'çÿÞß !½Ž.\D"cì5Õ툽ºKoQ¡×X©™{`¼Z½AŽÓÆÑýwC'׉×røŒðúfš†ãu¾ÈXuÞ[|C9Õù¸=·½–¿H¯né5õèq¼ÎW/ñã¸!Š|qþÝxMÆ,½ê󽦺=¡WPáï- ètc¥I³)ôjގ>ÞD^GŒW¼ll@ýz舽õÊÂ
{~'ç'W(96ZF'ŽÞ0Ü3šßó¾Ã´F}šêßj™LùëÖwXfÞ¦×ÿ'`&º´úb¥ç›y9.,g÷9"þ£[`¶•½<'?8›¹eëæD¨È×Úŧ¤ð^!È}–Pˆp°bœ+øN¦üÍ_7g1¡¹Q‡5ôx+üÁVŒrå{Ê]^ÏnHŽ}©fm7­:ØZ+/>7pL>aL´0N8j{m\÷º¶jŸ½xa%³íæÝ>¥ÂuÌܐ¸%ŸÃ¼OebLÀD‹Â˜ÐÜè£jâ`t«I"X'ٝ&C Â¹Ñ.ü`®,š:¬Dî÷Yu70L
ý™l¬nhª'Ô:kç¹/'âŸEYu–k&^ěB"¿"ŠUÂUëô¡ÌúŠ5Á-ŋy"ÃNúò;ÉQ
å‡.ß="ëLrk¤Qb܄†°Ò±ÑpÐRæå7Q^N6´@ãé)Ü-¥BDóŒÕ#¦£×ÙVÉ.¶0âÕ	jóžñýÖ¸_•W
4<ìz;[K…¤^~MLYNšÛ³¡7¯µ¿^+ù#9ˆn*ðÀçlÙer»:tÜêfY(Ek'ðÏk'¿¡KÛPxì9½&ý'Àî(MØN¦ÑIð¬ÄbÈzàŠdfDÑ°ĝ†"8D\pà­SD–‰Õ¹£Æx+K¨ÎŽÍ
oü‡ßäñéR¥1dv²߃ðŸWr'ÒܳeFÁÞlÖ+€˜J<ÓÈ-Š‰•Ùö²‡Å¬2¦ûnŸ²‡p<aéõÏ¡asžñzˆŠ¦×Fª^íðVˆ@E"X‹ìƒ/çct\¶£‡±MÅZ´øA‹–8hђûXËáBè¿:«x>màÿ­ Õ)Óòš2·$D¸,¼ÃPoœ±çó~®úŠô–S@½Q݃hÎãÊ]ý·Â»QaèûFç\f¹sÎÓՎ¤lHæö6(W‹µ¸Ÿ¸ëv‹Ê}ŽÚÛw‰· ÉåöDóPãjÍD®3àÎ-³"qî<úérX|cW"'™
¾è˜RŠI‰"iÎ&Q˜Y_aÎ(ÌğÅß%¯ê0¾Â©KŒÎ-…å 
¨ÏíÐ⒞ýgð÷×iŸ7ÂÙwf~½"¥Òž[æìd'öy"̶›w(U¹þÍà`ãöÔÄAa)'´›17²°ºSÍ¥ ˆ	º9ª˜{…Š	žQۄ•Èý>«nž›)¹0^.—ÐPƒô¯*Î>i1Ò¾«ñâŸEyj'7 65S¸¡"žŒÏûô¨e£yUTYù¾ž%<Ú/æ~`'ó#öäN÷w•–ï»%—ò­åàæ%‹'CØ0á£!Œ$6Z'ü¦EkZ ñôî"ÒÙ"MŽ ë1ªGL'«7ý¯ñNaðܨjÃÐ*·6[qęSµ²¢gOP IÓB:Êië(œÖh!½éAKH×X!MjDd^öÜÈȶN¼ò†®
é:­NÔni'!^šœ_¥°h Ö6hp‡	]-ÆOÖêT
±4%—ÆƵnOÙg[GÇûNpÍrCó¿6_‰ÒzÏGz€M²•«m.L/£káobDÀ- &?;ÞΣpåÝd®5­µ/Ñ>(†¬Ž<þÿR ©µÅ:M°¿4NQ`Mƒþ"Hƒ5ï‹´<¢µ¿ooCÐJ@	MCÁÃ!542:H^aÆÊæQ¸Æ7斡{YY‹hĄLÙ;¶F‹P¿ŸáB8AMçãOu‡!'ŸbÀÚÖҏgÊZ606­ÅF'™°šof"ª×ôP+/ Îc?4þËq~ËL˜ˆ×ÚÉT0ûíÉVººáÎþbÌ&®+/8¦âšª"¨aÝëYKb€š?ºw"ÄÕiBc +m%4
u§[…ƒoOŽ!•È×#ɞ‰µ¡ëØhيb,)·hÚyŒê~aìt?ú1	^¢ÞX¼«£ô½@¥_Øy,öóòÀÞ<v§[Í#ƒyë(°÷ÎbšG`Š &šG`-y©kÞ7ö…[
#r³¿¡yÜáÄE†¶œG>­µ2m!9¹ÙRø#k¯Ò9Ú\Sö퉭¥B
0CøUƒš ðۛwX"Éì»	±<Šýq‰tC'lèn,ö­á"#~"'.¥¤âçICüXZ¥°µxívÇCé4»æÉl»y·ãÖ›!î¯#&¬8n¶0ä>K[…cC€5´Ç6&¬=ފƵ¦4$¹ C9ÆàB@efªƒòžôÈüRÍÚÝ¿ˆ‡ZñzðG#ÖëyÌ7çü¶õ<2ȗM¤Ö[Šæ''­QdNV3ãc¯UŠÖ:°¥A1¤¬æ`.鍕&6Eô&þ#¶ög•«©€ØTj"ÏÁ<é9¯Ýª¬	]´ôÁnOÐÍ6{ÉJoOÁëHÉw;Åhé´6‹,´c"×é†ÅÝä:ÏrnѼà^Âe‰[b/&™¬ffSP¹à£gC@Üä\g,¿›ÆpØ-ˆz"ëÌ<jB>²u:ðÏkQؒ«ûvQ6Ý`6óp§âÑÁ*à¬çŒÚlhl4´4­	¸"‰"D[@IÊíbôÓÂB@MðÍQó9°êoæ‡X^6Ò._Ãsâ
}|>º€Œºn\áÓðÀ¨Ç]¡BãÉj??ºBƒ·¦+Ðü'
ßêðÓ¼+\Ç¢ñ	&§ËɘºâùDoÑ»Óo,zÙYÍç._$yû~AޞÜ~#wqqZÆÈJænP¾z…ºðz&S'
¤x¨~G¢‹ãß«§1v@ƒ¼¢Þ Ç)9æzu—žÃB¯±R.}/ðš6<?ÉóÜдcÛk÷Yâµì:{-—çݵ×$òŠ–åø´bÌÒ«¾íµüEùé5õè!+üpÝ ¼¾™¦áx
žµ~''#É9pý˜ò½¦º]±WwéoŒñjÁºÈ*
×´q4Ž¶_E^‡¯åX†VtºóÅߪ!ôêê閨Â!Æ+¼=ÉtoL¦µpnÃÈ?zÃÍøµzÓúîÞ¡ï- úÔ}éÒ09_
ÆG™Â¬‰j!bðï!ñÎÙÅYX
%úäâ¶n~!ÛË;["š™HÏÙÿELöM€ZJ"Ã%L@›'ºØJ~ ›
±¹	¹Z#®e V"ßM $¥>-XÀ¬£]PÛÆF8ÛƄÆj¥`% ¢"è 
PWÇTŠø£R
TêJ¤"œ	Tè•?r§Tùƒê}¤¦'ît`­æ&MuâR•µ±>"69Ð=‰äÃ4õÂd˜G"õ
endstream
endobj
43 0 obj
<</Filter[/FlateDecode]/Length 14802>>stream
H‰¬Wi[âJýþ>Ïû#Xd'IÀQpA–+ŽFEÿÿvw–îݝŽø¥ñ‰µœª:ujܪdʇõE¹hö¯Õæh³Ÿ)+÷ò2õô3S¤
V>ÞÍT^ÖùBåj\V›"^õÿÿÛÓöœd3µƒýšú"¸9C6ðjëpo/÷ïé4¥'+깚+Üì#‡'Zº[°t«ãz½««Ï¥Ôoð_ó¯c`ìÄ܄
Ƥ†	¸a‡uQ¸g…µSúûÒKnIÆ4ξC7½Le0Í7j.Óé'ð•%¥ç!r†f<X&ü$_øÞ-å}nÊƞó˜ítØc'fÜ_­m\áŸ{ÖôLõݪæ^fõ˜¦ô5>w(Xö°Üxa]yß™JÊh)yup@'öœgr[‡¾ÒÜäòñ"öʆÊ/lr÷1ar{ðI7ðgŒ:›Œúy¥(/Ç
GªŽæ¦:oì˜R=+nü©Î®³	º=ÉR•Íû	l¸ÀØã	°ñÍ/‰ÍU×kÅkèæçZöÎg
vš´µ'Ò#Ò,Oõwõ)yW#à›D/˜YC7^ÇëÉÓNÎùhÉ.èTߍq¬¤ Çá-3;YÕIt
.†Ó¥Ð »©Á¨k¸­`m8ÖÎÔÙºŸÛŠmšOsëèÜ4ÑܼgNŠý8Ÿ–>Ðì^v+
À½V`$—^L&ÄÆà'-lhÀ·IX\ø§žLzÈt²h^œd°Ú²'kƒ¿_¯ƒ6Êv'Y@'Ø7èDŽ]'jEx-Šçâå"æïL~X3ªñȘÎð¸qc' á°|ôO†uÕsÊ'WCDÿôxú¹'SÆí÷dkè͍¯ÁÁ΁ڱ¨¢¤ûkó™'µù¼µ@)
4íKAÓ¿´üŽ 9Öi7u¹ØŒÏÝ^þÓ;hbøøȧÓÀ BÕ÷Ëævã~Ñ`Œ}J_3"&uÄ-ecšo†Öµ"mî!–´m͹8çšúæÚfs5DðU' =%
ïì9_WçÜÕÕ<	ÂÍ'm"-OÜrRrkMjh?,êl>ìV%sð¸o<¡ÃԚzõv8·.øŒÚFD›Ä"M	Døpx''ž)$Rnõ*kÇqÚ¸dá3ц¥'ªêòFäQóst#'g"}'®<—à
Ÿä¸N&™%x°Ö1žä'A¤ä8IŽPçü\FrÈAU)u;RmጧªÿRÿdÀ˜Y‹_²a	câ¯_÷ö"
K}Ö¢Ãð1¹ÔI‡%3ØR1¹W¨,Ù ú'l¸'S>^\ä蓩å?™<ì‡)Î홏—¢·g¾=Ù ½¶<\óÎxæ?«×+Z;Á½8hèq;M\œ–Ü%9(na~ùÊàgÇûóíäÐcڑ3—)¨á‡ÊÍËÍÆ~f×Ùo³·ðfŸ¡Ó^[êsòãVÐA6u¦ˆ:9¥jmèݞg‰[)l%jNpï$º6IE4µ'Š±|Aéö*¥ë5'ƒÉ»o¥¿zÀÊ
¦t´dÃWêÆpÖvm؉;¢íWäÛT"á(®N)òe›VäœNw9WŽ£Ú"º)‰ª$ç[¦tr¶€
nÔR7BËòpìޞ°ðùÝS*›Ã%«} hò¤»lû·§äÓÊbƒÙ[€M ¸†èÉ5´o'YÚFžBŸ"‹ÍøÜÍëöÆ·ù¨k»üXñª³É(#[M¸8­Pb>KZlʽ'ùkÏî
'…®wï4€¹p
%;­l^¿BÌû;-Û
%eY- i(Ì䞸ÈЧFqË
¸sé¹a'ýíôméC`ͲbêäY£E¨:›ÏR¾E—Op"û7VRÐãÌ£I°çq>ãK$bºoû"€Öö¥ˆXf\4oÞšµ!M²€*~ң܀ß=%'†³¤9AÓW¨q¿h°fÂ™˜"Pmg¿J^°´¡:µJÊh‡Áw¨ASZûbw¼‡÷œ3
RRf­hûÕyCÜ'†ŒË[Aµ	6Äù¡ÂÙ@Cô<ê¤!¥šrڈPÎÜyƒâc·æ¸U!:íªë­\EFéCM¶=àwpÅ÷ä<÷ç«PwÞ7dÛvžGÂƐœÆÇo?'Õ!æ¡æ'#ÕáfWvŸGhÍãŽ'®m(x}Vk
Úu'<ŒÓüóBøÛÖª¿‹-öhSdñæˆk珒à,03p2.‰	šD/d6"èÆᏣ%§Éî?ƒÁi@õibÅ"-~€)æié5´Pÿ0¬Bªn§ùYkÅC±ƒ~!9Š¬à‹à³†ïá8ÊFhh¸Ü9/{{ÞÈ,¹¼FÔrÈttÏÊڞë~Îé%oÕL¢k"S´ŽNU¿¾ÀÕϽ¼gNÁŠo)eã›G0X׊oÁïú⍣–¹3ŒØ
1£•`IiÀYæ$š·0›&­'Ò>wb4×i"›¦Ói1Ÿ5àpXçX{‰÷‹Ó¾(°ýSƒ3žÀÚBb<c2 UJÝÎݞ£•:›Œúò·'gI•RYÖò•UŒ˜l¼°/%ÚBN1N-¤ýnÀ¯¢1¼bÔ«·O\\ò"°y$¼`¸Kº–Õ¹+"'½¤9yjÑjž'&¢lJ{ã×X{ØTÛA>ŽµÂ;7°|ü¤}A*Ž5	eSËIìQÈÁ¼
:ÊJX³M1¸³:®Á³P»ÆäoZðºðï
<ÆåÃÎÓ¡S"kµÒ×qà&Ž™Zä UF"—ùOøœE2ÿd[¥Þ«ÁçW6QŒ{åKø@sþ5ZEá†:Ȝö¾½¬,mo…½¢†Žå"à/[¯ÙœuÜ,DõR£šë¿%ÕÜéífµúM‡Ïß=‡1ˆappÔXmÆÙ²A(¯ÐÍwýO—dÂë·X¬¿ü{ÇöZþæzµ¢¹æ»o(Çjãùò†ë5¡µFÿð¼>'^7q츱Ž/«7DºO‰D{µb/3̆yÂåø«—«ù—òšb¯§Å)Ou®WµQT/9^¿Åâ½Wý'币é>pÓ [¾WS¸^"³ÔÑòênOª¡"Y'׋$×ëÊê—#,¯À
r9{8øI•vVtý£9ÅH×~?½Ê|÷¸y}£È†óé·ØÇ£q{hòðÅé>gqVAÖ÷?|r"Í8õŠö)ÉՍ͊¿³¼Íǽ¯°ŠE–餐r±Ÿ»{ÿ®N¯ëíÓUj]×á1Ö Tsܪl	(ôLnëÐá>GŽÝÕi9ìÉ^Ғa1,ˆ	*0'؇)µ@ñïF©†Áàw)£í;qƒ Js¡ÂÛ^\>·6|¨ þ$TTC¨Nö¹˜·ãSž€â÷:›Ï¬˜l-²«Ô™µø*Cê(¤šáäà‹2"š\<7rÀØr☝&V-{÷Ess¢qÃrÂq.˜‹º`/§·yë.é/¹4¾)q­Ó	Ôdlá=TÖbq+æj4ã~	>lÑÓ³"Ûÿ15˜ÉU´öM6ÌÃ6 ¹ƒ˜"rWg×ÙªºoXH›×¯Áy%ì¼Ø½ùhà1ö@ûLJʒÞ2œ+Él'`6t{R¥ªçBaÃf´'œöW®@®)؁֖dšcm¹%M¦ú‡8ki²™4¼OxcŒ®/ð8µ7\RÔiDXù¨L1àãLáu2ɬë$Ú!xËÇÐþËÇVú`·ÀK¯þ.¶Øi*UĂ
pƒ~zˆdHÐ!é^:‹ã% À»Ž	üm%!Rà'Ô)&'tœpÕsâ$ƒMù*lƒ†¾2ŒN\dòãÅñÆ·N(ꔠZ
¯iDŒ—·œj6urÃ*F[.PªS
ø|‰ñÂ:ód¦"Ö4}ôÏP£MR\F\Ã|e𳪆À
¯Œ+O±íÜ«--°"5m¿:o°L¡†m-tã‹@Ó&ñdóË@£™w'k4»í
šþ°©¶ÙyV\S=¼¶"£²­ÿ4w¹x!Ù¸ÓÕô+G¾Jfïý&÷<%Ç3ÐÆ¢x.ѴƚotßüÇzu-¤Ño	5@'JÞ0(Ò® 'Š@øÿ»»Ù)ˆ/1g§žsF5âo%"Ä+š]H
#ëÓ5Ón={šìHF6<v—,%½ÔÎgärŸ†=Ø/Ú-TÚήt±¿¶I5چVÑUVïRöRšÚéD' lfd§Ÿì¯‡3Þ§Ôæ(¤ˆÝŽ'ΧZd¨ÓijÅÒ;—VT¥éû­^T½ìÞD]åÔ( ×	ÆC'¦óÔ9±úÔk"6Üeْ4 f°–1x'í,}°,›ƒ‡BÖøSe{öqªŒ1mY¶"-6S¥Y^
˜êE³àîEC¡óI®™[ƒ»ÖÐ'ÜiÈ­?ê*¸Îžò	svª•…¡Oê¹Ñº5×O²¢«%wŽAüG
Y"¤ˆ<é¨[zªìÍ×Nm·ú
&è«¢‹¼ö«…)t˜Ê»â´Kæ!sÚ-P·>œNZbUÒa	<L<nr!,ë3Žw%ª5&¾sƒ‹Ð¦Á¹ÑŏA;†Î€ùtܳŒËçÁqîMXuxŒv'RlÛ·Júæ­ ÇHcTà1͍Ü&FR07:z?™ÄñÄéøÆ0AÚá5nhXP²¤Uóܱšÿ©jÕ<¯Å4kAHPU¯æmv"V@¥ãm·8ã,¾€‹"çd[¤{7^ߜ.(ét3H®ÂbTk6'ÃâÖ°ããmŸypÖ]ZÅ<Š:í'F•
?ß­ÍC'¤ºéÇÛÔ)Ð=k'á1°Zȍ–85‰!˜æ&ìi¡ˆa'¹àóùc|êR¸²I˜^6Fï,:ùô:Mxøåªë[ëp–T͓ûMž•.Äóз±5¤5è
"nÍ¥²†ðÂNC9]Úi9"HÚÐʁoìòÿÒõ…
1«³'Žù•¡€
wbAZ`ê‹FւgYӚR‰P'i¾c.ºx3™ Û»œÐ•6'¿'~È1`SoGdf˜ÍWO˜³Ó*è'OÅZÀDYx!q^ùñ†r|_›iÍsó1˜ýþúb–A|'…ZàRy¬YÀˆˆµ–×kd-ü(sþà¸P=¶:+êcÎ1Ô7o½¥ô†?Qø
­ý֐v™zø`åÌŇ{IHjjŠ–šê߯"êsïk&)"îi™å vóÔ_?ùaÎ<‡úyÔ
£²xÀb\>ïœêyICŸ;Ðš­	ÒbšÑ<Bk;¥
"	:/—êBÿÔ<ê¬qkmèÌy<¹âbC—Ïc_™G+Z³6d<Š½ê?
6ÈÚlw¾5b*ÂvT}€"$»gGÃhÃ
\¦y"	'îüpU8ÙdSGg÷˜öhWüÀc¬õÏãÅ⏧b-T­]¸Ú7|ºß­ë®`š]Ô
9§mc®Í±¡?»,\¢ÈÊŠ	IÿÚÐÔå-Ùp‡lkƆ´KdXmˆÍÒDC«¨&¾9U4ÜhP¹à³ƒ'•´\ýf;ÄöB,¾Ø›ÇñV7ŒÒ1ðõŸÌ#ŒëY4Á4•:PӚ†ÏÕٌÓÆ2S#
ò¬JܞN(S[›aª­AS¡oãÚ@k/ûlÕªeЅX‹¬
ã]‰jÍÆxˆ mÒ®ÿl÷"íÛßd
ðPÀÌk¢4ma©'OÆmµ€¥hÔ)ÆpVtŠ¾íYžHÑ(×w¶3QŒjPЏñi' hJ" ty¶ÈfVX9¬tšSg
8¸7°¶qY%M¹t$ßü™YÞÀšhC@ÚS6&o×­xt¼÷›ã2®&˜OÇ=‰¤íX3àŠ\3á@¹-°ä°¤É-H?mqŠ+{ÑÅ\<Önð1Wš ñ	*?¥$¨"
Xôâ4ôœSg¤7Á{É.ÉDG?ËÊ»ÔUýaš¦«~°µT¬äZJç—&­œêÚL˜ouú˜,£ïI)4%GCþs<Ïm·©ÎÇ'ÞV2¡èãC؛rÜ㟹ÝU‰é¶¦[Ê=d<"úGyG¥w*˜\f˜DjcnÓýX­A>¿ä@~ˆƒBµADPXÔ@±€Z¹1µ¯Åh~ÎßÁCnù£z»÷èñôGÉ=xôiðÄö|àeæh'ÑHX€q‡Á"¼`R§ÛÛí6ÏmwÃub»}÷á1Ûý8Jï¼7¤:âv½×R³Ôˆ-îú/Oo"ßãZ®hâ3ën=+ž÷•Ûáˆq
ÚùùÏ]ŽÄ<ÍÙR¸¿õÃøùí~BíٟHc'Ë"p–B*SèvÝÀ5…¯[ë"pBjSÛA'v;Š}_Ö¨@vœ°º'~'ì\¿3‰ÏxV—/œ,"´b;ÙoÀäväÛnF	÷(ֈO`nyï(d«YPXü«€b³ñµsŽ®gA¾£È©MžIFπ+Œ)"´mdÐùþÍx»{«8ל³:¦#¦Ýè/©AÑ;Up
)Z'CôP¾ÛF"
pÞ>—{Êuå(Öww‡ÞU(¦íhPÌ¿`}HSÿJ±u¡Dù7Nët%­\¯`êÃQWȟ%à1¹)B¡ï5j‹TȇëQx÷ðbßÞRð®¿óVи•#ˆÿwžDè ‡BÒän9÷Ãÿ(ù¤Þ
#ÍM‰!oât=Èc-Bl@<óÿV›à®Ê óµ®í2ÕÇLjbŒø™ºñ)pò‡$:FõmêÊ%åo¹€ò!œ}ê¥åeNù5Ù[FþÐ>Œ`Ñܟ€+&ýø:½VŸ^̱ÊïÕGËA˜sÖ¹mÈ@CN_øe·ÜÝ~äÓ=
>¶îüc¬q´
,ú•JðyÂÅ(ÄÖZ'SַՄ´'¹b1ÃǶë—
ĵžy®þ°âáÿvaþ·Nô•'¿7¨ÔI›ÈÇL`õ¯Ÿ÷ÜôÖûöö
·ùÈR…Ÿº…¶z»•W\™k1?'QÜaR†X좯mǢŝwÞ½/¿&)y÷"¡	!¹»aæžuït©\û>ÇNÒdƒiäúTÝd³fe‰…y½ù†=ŽtÿL¡Y­ìõ™=‡$EÌÍFáT¬^û)/ß½F°
RßU›`F‡Gþwõ仑Òs3Ȩµ"2ž«W^õmDñãÂØ÷\
Oê7‰fõu!†ÏFùhb>ò-rïׅfö3ꌢ‡	
öŸ˜ˆ¥ÐEƒD*ãŠBðpê?Ò2â"Š¡;ÞMCòÝkXùäìŒP\Ftî hÞ¯Ä~ÁïK%núG½0©»c˜hyÏxw*Eæ
ÖëåšÉ÷…R¦*§£¡Q‹k·5ù!¬å)ì­Ûå!B>
"¯ñDÝÇ[]KXÓ]Ê÷ñ™¢ßí!Öb—
ÎÉEê–Hȇ'CãÙ#ËÄOò"é!Þ`ÓAù¢ƒðq,Ê
Z'Ý/¦6:-ϗ:ë 2î
{ï¨\}$)ÑÑbáfz[æ>ƒ³‡û`ãÒÓòeo#FÒýFõ¸з<æf{µx ÊÊNWYŒßHa¢hª"ºé—r"ÕÞ«¼¿x.ˆ~– ²"R´v‰H=ªÔRª¥–Òj©Ý÷ï܄"¢‰åýÇ/‹Ìܙ93çŒØݱYž÷wîãð/D³nEï4
 }æÑ»³ŽF¾ê¢A4XÕgm[Ó¦ŽS<DÑ÷-
m#śv)^0àÕ-ƒLNj0ô
Èî#Iå#ì:ÛÆ¢]	K׎PTݛ€Û»¨yÍËP6AAÀH~$'"œz‹8;Hûø*I;ám	ø9f i$S8'#Z$hÊÈPM0­È®`òÓdÊt-Â×ñò"'j·RƒÄhêi%*d±&–Ãߔüï5KKʖˆÄ÷Z"N±]¬N=ý«1§ïªä0:>ì5ù¥8gÈáó41NÏjJ"KÛÅüg$+–eŸCþ(̋X"ω)óÝ«'<›E_ì* F'üžon5f]äçĺNÊú{sWÀ+©þ;æÑ™,ù¶õçJ'ÐP¨[í×$>'p«K="O;ny~.¤üc¢¡È~ØÓ|º±ëzкk¨
ö.¼7™D¸ÞoÊîbk–üˆŽ:fM^‹3BޛõK!-öÔdR+
7,…0ÎЊyC/óãy¸' DY<:uöØCÙb""ê}IŠ*¤Ò_ÞÄTôˆò¿Ÿ¯¹"½'Ö">ùK_d·/-þœTî¿ŽÜìÎy<Tâ°±±¥"У?2täÆRô«Ð-Âm͞'Ámz<s×" B8r³g÷[öÏT†´Gn:ÉÂLÍ]ߣ®LҒºьÄ®[צp˜Ð+çáÿq•Êãÿ˜¶ß>róg۟2q*½Då>
´¦4e"Õ
äû¦Ûþøas0æ"çžÆl"`€Û#ªëíRzŸó+Ý5rsÆJoF[Å!ãžCnNi;³=‡ùæÄ)o'ÖЖ™Ý:­c¾¹€"±JkGJ™­\Ó鶰
7aÊKä)•Þõ­íl±'¦ª8ä氐39b`=¬LQ/uRø¦PIJ™86Z¾LJn^HU¥ZNä&|B|/ä9Îú3"7'ò‹²hˆé@+—ø(O©Y£"÷;oyÙ~Ì'<³…Cj儒´ûcJÐQì&{:¼üŒq'Û7« 7gîVÞ¯†¨T%JM#zÐûn¼Ý	dÌ&£³µÐ.°ÏSì×K_,Wª³p/8 ø‰þÍ4]̦ÚmҝzéÚú8õ¸€4\‡«q#	²A¤š÷ßFàf];H^LëP"ÿä[]cžC‡ùˆåµ*Ènw¤Š¦{–ÂD83(šS6Ø릲0'ª€N•"&¦;†€9>·H檨Ò¾ŠæȜ›Møùh͚€20ëÙüWz˜ÖÎ!*»Fn¬¯և-&'³Íû
ÿ7ú°EnbSÇOöäìNý6ߏþ_Oab°€:ȱ¡äkfÕqÑâvâ".&)HÏÝåÖìњQ=ûç
ÐZãñ!ˆÈ$@?	‡=‡o#×"'å.‹ˆ¨"Mxñ{1ír#ú©"Ð-¯"œc9$Û»þ2|cq$Çjüže§Ýš½føæTדd¹'ä¨.»oȹ	¶Õ©öæST‡×¨?c606‡¡ñžšL
»†hÎWé_Q£ï¹n‡€4#ÛCôºÿð½C®ËwwÑ1×S=täÆD¹OTVUm™r­#·ç)Ù7çÜXé³#›¹9÷`19ÓN@Úހ÷ moŸ5(+}vd"íAÚÞ>³Þd±	Õ­á™Ö¹¦7)_P%þ'"‹áò9'}¡;ô)×ìfà–$¸þwƒ`ßÝèmÁ&\·®<A·>n	®ò–'ÿ]®LÜ4#qð‡7'þÆרP‡/y'
â+ç9kjgSí!7‡ŸQäG_ì»´ž	ÉÚ²Ö³îCÀ'à:¨¶¦[- ƒ pÌеÏSì×K_,Wª387Eö)ZSTç.­yæ%jspÏ:ܞæ°oø¿µ6†€Å|¼âîPúç«þ¾÷ð¦q\èxŵºâíØï&èmeŠZ‹Joôa&¾Òøˤäæ´ÆÔr"7áâ{!§Èq֟¹Ñd¦"ã¾g¼²(AÛòæð.³k'Anþìx'J~¯´YÒQù®ØÈW 
±J°FIÏíÅ‹­—ì-'ý›FÏĜӒ6ņàê§úZv–åfC(.'<'üãE¦.–Ÿ¾ßÌ®QøJiè*Ì¡d|Dp¥Q\"%Ì!7;Qi†Œ"Ûß&š
_!C¬2'¢	†ïiOÝ{‡=rsáêãÒkªó'ÕÇWê¶vÉêãÒ#7®>.=¸¹lõqé¡=/[}\zM@]°ú؊6.X}\z¬Ó.Z}\z€ÀYª…?[ÄY•þ'.&ÉwÉ×$XÝ=¯†Æ½#œzÒ6c 7å?ßÜÇWëNÖ¯ok¬ž8±`Úñ­7-¥º+Ñüî4úÂܹ¯êÜ*$ËŸ~Nü¹±Oˇ•ÖÕ¶eçqjX"œ/BÆ~FDk?ë
öI­¦vl\õÚ# Í`Ã?V¶m\ÿ{Õm"T(ñE5-Ð(¯7#
)Ð?Ò
ïÉ÷(ïÝÛ'` ñ3Œ´ö"Ñl¬Ð˜wülªòœï«Õî¯
¢^¶B^ŒoÈHŸIT™6ÆzáF=çã4âô©£S†Îä(­‰Ã?E"Ñç%
—nº;<|ÊÁQm𢶑›J¯Í31ö¤P"¶Ôl&Õ^íÙ§:ŽbÝÛ¶ùîЉ¼›Ê=^%mI€WBͦoþê\õý/ìúqŒìcHš–‡Äµ!W¢µÊƒÏ£çŽ3Ða"‰Ó' ÏKë$ԍIX¾æqm´<<oæ;œìõ:Q (-	íx~#	¡ùjªÐuiZ´²ü‡¸73×Z@¢ï×IH7ܶï§]`@nt<à<À â5,ßäZ"¥×˜‡÷üÃ>0ê°U-|°¼lê 
"W6L0î7$pm݆Á@ªcvµ…VA¢Jß±GBå›҈̣A"\sííoHÚ߁ÀrŸr·ŽàÀs
´L`¢9dƒ2ÂóPŸïkr
cs´ãl±yä°¡Œð4Ú0[JÇ&D³ß†1m:6÷—4Œ°u
0WÛ6ð<ZÔ6qÒ¬Úбy 
¢N
kxòi¹ÔYÙ¨6ÿGë䕲´¸ÖØþŸI¤ˆ‹6;HûecÒ̝Þ@Úq½O[š'ßü²a@ÚQèHÃQèH³È>¤í?Ä/¤Ñ&!AÊõ'fC˜¿m`vMA-if"Áè$méF'f̽‡0bs[$} "ŒOClk'i$ÍKÒx)ë}÷@˜¦9ãº!Ìû"+|!\·®èöݝ&¸<́à"ø¤»›g‰™¶öEk>ãFàXO¿';¼LÒN~µ=^MõÐJJx¸EW¥‰—ûüŒá½¢é=º°s¸ñç­?ž§Ü|Ë÷ÚMJ»úî1phZuøANY¸eµÛ23íÒn³>ÍÀÇShÜ¤ÞÓ ïñÿãşqv[MƒO·Aí¨±ZaŒ!e
/ڎdô?Ö«¬)un‰¾Uß8 C™ˆaHH@Eežœ@P†ªûtûí="DŽz9z^RI:Y½wïÕ«»mƒÎ;%ß©gÀm+‰ŽMõ%r¶¡"ï
H
ÿB­tÈyçvméœË°w)`•"!˜^eҊçj2~T3u<V³øþˆÀàS59ô	âò,›pñ)=‰£'1ܬ¬á"
bÊ<¼ùàMã†È‰Õ®*–oæhð¹…#8I k<0¶/ØŒl7#8ýX‡7Äq*xXëfªyv§g4ڙպ46Ô2û®ÑÚÎ`mKýS ¯QÀ¤5¯a±çñ본efƒ³[£4M{(¿Û-Ù¦ì­68ÿÎdŠ¥'Â.†'"Míqd¿Í1f"CI…Gá †§É"ºH™>iIòä²ÄÂ]W–Σ~8ÍÉ@ÑÎJ
œÍd¬ÚwÓ 9¯a<"œÀy#Î["ý}ޕ컁ï‰Ì\jt9ó©ê2<êвÝeT~³scþÓ¡š«ñälÀÞ£Ý<ÆÌJ~?‰£Ð*4ãÍÝBš»:ْsA‹Ð^ÙÔ+á¶%ì½ÞQnl'lÉYîÆ2¾Ã»ÙNçSP·Ú¼{Ž¬HŒnfˆÕ'§
Þ[6Geÿ–'50ܜJçV8
çՏ…V1wђNà±¼Ä(È
ɸÈMjU.ŽçGЭàÇ2Eٚ9ö6Džž¼ÕÀ^ž6¶ dÜ¡©°4oP"Eoa¹è{ֈޒe5›=ø©!¡wB8¿Úd÷MÀl•­ÐAòhþý¥†2èà½	ì/ÈvÁ"µ­ö&sÒrd+ïEK¢ÌéþWºh-‹€¡aµ'¢"‹úXp˜.s¯ºnŒóÔJú]ºÎ3ôA¿ì^…qâAA'|Ň3Œ±–­×*:Wp9mõÑ<7ɚn°dܑ.ä¤n6ÿ…Ó;Çc¿âÑxü—XÛ-fëÊúéáiù‹û÷Ÿä¿ÿˆ¹',חӕ¹žÍngÿÙ«»ÝËl¹ý•ø%ænôR)5fw«éý€ŽztºWžî"\Ý®÷wؐD}PÞ¸?³æœZzlÜKm͕¸¤³j1íáÅ`
×Pmžò°W3÷ø¶Ñ½à	ï7®Ü2<¼TVP!e°[Ÿ6e¬ÉócØK'ŏÌÕiS•¦ŽU*g:n£´ô$ǽ^g/Î6Z¼˜j
æªiÖ½ŽdtÌö­™Î¥ï°Q7ªï55,ˆŸm˜n)Ô7Q·{xny¸Æ Ëo¶<?ö¢ž£KÒÃçÔ*l<0ð°OÍÃ/¯{¨‡8CÉ¡ÆK³m)ëù‹sì˜yà†oì{é‰
¦ÛQ;‡˜¸@+ëõ6èQ´³·Üß1D¤f›9nB´-½NDLüF'†öŸ¢"¤j¦ñš·+w"quS†I؆DÈÕ ‰"mÈrnZ÷Ýr¬™'ËÐß
²¶áÒÕ ¸ý[	<DZn×V–ô&È
î\Þ-Ó)ÁˆaªºuiW«"!'
#ÝA2tEÚ8y2ðmḆº^
¼È"Wåñ5ï.Õ>¨¡L½ÈWw1]AÉö»b?RÜ»Ô:RÿÚfxß9pت°±ÄÔöz+ìÝH¬/.)‹;cÙ¤Ôð¹¹?b^"×(ðñí/"Úˆä)~"n~)¹ eñd"
דë˜V\åNûS+ Âvn<NïÙî:n¤úR©á7»›ÎíÝ79W§aӈ›MDÉè"d'Æ]…f"±¨+øÜ(Æ®;À
¾R`ÇCz§< ŠØŒŒa'‹ ;p™(+e¸¸"ÐpW£à#¶õh/§ãn|FÉé3µEö‰2qífÔôè{­¬åÂC(W½»¿4.JžR6PÀÉ0‡
Ùû*Fʦ•Ä¼êߕf¶×¾ˆ7¢"z"d7JïŒñÓþ;•~×xÉ.§¢ßöMcá½CyS»í>ÛDB˜'ŠôhçÈö5F@—8G¸!ˆ#gÈJz4ÑP"ky›RçRoŒ¹ n¢E-æ×w ɳ–q2Ýô¾Uk%ú•ShæËçyv±®fÅm¬˜/HÂm²s¹Ô¬E£ÕËcž	žžlÜßÒßüÕ^æ£F†ìæ¯ö252ØÍßíe>jdHÐþj/óQ#CšBÜË.½Ò!œ'|(Žªú;‰±ƒ>Ô(JÁËÍz­l²Peã¨z'Šˆ®Lä¦âªâ^=ç…?k[ô}¾¿O½Ç`1àž
aݗ)à…Ìe…9k«Nǂßy½Zƒ¦þ¥±^§W!¼a§YÙxMӏ1ðÇÒÌZ­jŽàÎ&ýļK1èÐqzI	€£¡Á¡Sâ€e¿C´È»þf¨âvÁžè†['ô4o'd")åáz²Ön½Ž°}Ô»x‰!yW)KbeæE†ö»ð•ƒû-=†²ÍÐÎÚ[XïFiØnX&ÓíÃR#ØdÁ›QxiŸÍ΃¼zÈ9D6]¨™æЃ¼¶á".gQ¿rÖæ–NÐòìn®p@û'÷¹¡
›àÓ¸ºÂ+BËY8ч…Yacs³BÏ"]·'ƒ€Ý¹âvÅ¡»V'v²VïLvþ]N×AØÚ‡Ï‡Œþ¶rÅ¥'aõJ'@å³ €' _s'xUO+se'IÑáw˳$ë|»K¤"Ɓ™øj½OÈÀ2®@úSžÑG"ú€še'B_Pø#|Df|•,Ö~´þpó%†ðӍˆnéüæF¤O©u€êÍ'ò±Ÿp.^›oå9ú#¡@bó;ÆOņãH'þ£áøOñŽîEȂÝÜî1"#NDÍ^3Åg*ïďøM'vôF¤o&'NC>&_ä§Ø±'É6^ëB?šr>õ-Õd•~j¾(ï¿;†%ξHЖ%rߌÍà%.¦ËVñ–,â· }H"?وôQ4IЎÞÈwÈÅ4Qùaî‹êQEºI—õ0ÁXkQõ†ò#"EZáþ0¾^ÄgDaכ¯'¡?¤…"º‹ô÷DL9F€>)ÒÚ+3½…©5X4Í9ãÄ«ödÞfÂFÑ\1vUÔÇçÏÐí]F•|§žÑŸÆ¢L†¼P®—{?hV"!ã†3I‰þ	õK:…¶æ¼2,N9I¿ñhˆõÁÌñÈ£<ªÀ(è0(\¹™dhü£¿5»'ÇD?ҙ6šåÉc3ÃÃnPõ¥Rÿ£½J»›È•èwÎÉh–,&ÄÖÚj±"ì‹™¼Éˆb×÷۟–*IÝNöÃÃ9×­ª[¥'T¥>XÙoì¾ ÷æ>Í=)ï~³_¼ižÈùSø½yñ0Õ-Ž§G©â-=	ŠfªøôìcPD1ó`ýŸ$̈ÿ2[-ï¢ýËéÄÞ|ÅLª¸|lÀKÓ£f—•·'ºt-/¹]uÃÔð®ýÄ%­í¹‡ó݋òjþÅû÷û¦†Âm{ÅÕæ¡©áé'ÛÆÖçgG…Ý霗-ói±½Õ2›,™/ïŒø–:óàïöŒ¸Ë[›;g¶3¼™v«¹ÿô¾5˜6š]ÒúP΄¨æÀ|NæÍ,µŸN<þt>ùvåé²øRû2œÕ«íW¸ñáÏaÛ~­Ù³÷Êf©M–ç‹ÿ7eäc"³÷–Ÿ[MÞØ(^ébuenòôÍÒúɳ»îò˜uµéÊ2Û,ìÂYÜÖèì߇óýáP"¥š0=
Wàh˝ÍG¦®êÜíÍÑÛ9Ýnš¯µ£6¡GåzÃüÚ¥dCŽ[í›ÕëÌì×Ñ!Ç_'Âq¸ý%­³×ŽrÆTý±9ýgíøží÷˅9Û£!£#6ù¼œ…ŒÎNx¢Ø»Ë÷ÝEa›_Ça5gÝÜõ¾PðâÉé^ããâ?ùÊÖB§¸_Ø
3÷-銶ò½CN&wý'â›Çìeãé%Ô°×n†¨Çp^z{"®Ò¹)óëâ¯íÜýv«é}}ÉÞ»•‡Ù'êÝ͕̽ƒÍqíÚŸØ¿RdcuZšýú;Ÿ^~×^›Ñ&÷]›Äv:Þ!-±3éZ'Ù›bzZo×öTµ}6íÖB{Ïôϳ{ÍÖç{ÛþR©æM6'É‡¸n¦eٻԈ-‹®=ø2ë»ÀÚ#Hëýûÿ§wöb¯5§.®æïWÛ¶üe-«X°IŒ‡?¯­'XÅ¢'Ÿ׮Ϲ0½Ù¯±Ëùçzén—ôìœk
SÐIg×[D½xÞ×Ý.ÉÒÆÓbL¶â¹ÚóEÛx›¼úì¡[¤ïiö>úÁa2ãÛÙó©¥o¶"µ "©wk‹gó§¦uŸ˜â®¾NÈḛ^柃GË&ÌÕM	Ÿ`~Òýåó"7§ÿö–.Ž¿wOÏ{7ÐÎiïû¥3'û§Ÿ>Ÿ—‡?OMÿ¥™ÿGÌ?ûW録"cRAZ´4/Ï)gÑFVڻߚÿÖ[ú|Üû|q~øígöØaíÍòíúRö8óÖûÆúI6er"ûÆܨÙ#kh3Ý»C²yû§ýÃþ}m3Yµ¿|*ÿi¥
#ÉHSóÍ~d"d›Ùîß$;36ÖM'¦'S¬ÉdÖ
€d…ùÍʱ;BåFG¯ƒÀ­¬ó`ÇÆ·)5¹ýO˜à»&'Ld.úoÄÝéo2³¼?ÆUJ궘ÏXM³‡c—EÝ7³Wõ7{XvNy3%÷òÜUõöŽ9WfûiÊ
ÈÍì5ƒ_øØ'ÑZDnŒP7¸ÅÇzTO\÷ÚcYR3¸Ñ§ï,öï>ð&3$ÓE³jä€Õ¯Œ€ˆ3Ñ´w7±B¨Jv«!
í
ÚT#¼Í	•ìPð6C "Ô#T%¼Õ	Y^?Õo3DBɜ2µ¨Fx›!*Õ ám†Ø 	¯F¨Jx«a¾þýöuKÆÑîõ³à—ë·&FŸSùoÜãüfÞ7Þ®NüšŸmÙ?¤©5×Eá&´ŸÒíC«øb¤cÔMc¦måÍ­`xQ˜Ö)R&Hž">cóž	×'2Ÿî
¼F—ËÕmEI
bt'阁b	"ăةúW?|€%sFl½DA00gyŠ"	'G"¤H§g¨
Œ.—A
B©;@Ba£âT¥HÉ#BS¤ÓÇ3\AF–Ë 'Ê•QÐ0xÎ+P™@Œêôs
W•Ñ&4ÐYaµ'	§EŠ")hDXŠtúx†<+£Êeª"ýè'yèbI€2ylêÞ€Nc¸V:Š4)cæYÃðµÈXÄÅ"Š,ˆªïp‹ÿsÁ¹
Üß)AX¸"\W 2…Šñ
Ôéçî>Œ6¡^®CAãlç)R&ˆŠ'T¥H§gÈGƨr¬mš‹%ãL+'X'˜Ó(² vª¾ÃöÉ?|3 ÍËxã'eTˆ
.*D¯rùÊA"APßj8QMÿ1ÄD"	@9èâ€Nc¨2Œ$ÝÚßf5—)RFD&O_">ž!Ý£Êe ŽàƱù¾ƒ©Åiž%'ȐèÔ9†ì
#Hc.!´y‰RœWLÊ –(†wª7V8£Rßázß>À'©vå";Õy"P 	Щsµø'¤ÊÐ,
žçÒd£rMsŸqa5üC$c…ö)ȪY^dœM‹ÄæÁyîÕV8ö7"hc‡j^óæ'ý4Ó´I¥!îš%ìNpæÔºæä¾8vgÅxhùnÙMd
	i`ôׅëÜ«	Ԑªy͛Gvg²""¢{ž²c±bp¯Ö5ï$w¿œ8ܳ'ÆKÚPö£Ò»Sá!£`àÄc;14¤a¤ ETpA¤hj›qä`¤ŋÖ%䁢FQ]ì|R™~9š
pŸ°Â'1—®S2WK³(µS×ü²Ç/KSô®Ed-¼ièÔ5¿+$/ìÁcZ¸ÜA`'(|9Ìi5BîtÔÅ0"Ê•ÒkxՋ£3ô'"ðÑOFå
C,«ÑU/ÌrÎÝ;‹ÙžéÒ™@IòpšübÍ#T¢`CÉp–¼^wi0÷2‡ªos"»¬yˆŽzQqOsÇ-puÄÅ8	s°o¬ð©
‰?¡¸®äAËRW†¬ÎÔJ˜CðÓ"°ê°€µEêr…ä}ÿ²UaióåRù‹ú—¹5þRÚ~ƒ¯ð$BlÀ<'þRF'œ¥¼"¶à` ké`]…9؊á¦8‰B¥á\æÞOøÓS9ÜÔÊÔU"«3µ'€Ü'Ÿ'Õÿt¦´.!t¹â)Ü:	Áü=ÀLwöy˜®®ýPRŽNK¯WÏl¸ôC
X€%œrBNx$ç)ƒ¢F®×e¿8Éò¼,ãªüÕCJwג®.êi՝Fvgîe<<Ñ[§ì:YD½ªº'¹Ãr"›"0lº°"ŽÔÈÏ»ãN3ÎDZ# Içâ@`TÁKþŒ'%¨Aºœø*ßÝa8ñ±X"V'-
³ˍ´NÑ÷HˆÄq8T5Jx$Ä<ÀBÕ)*k"²ŠÝ
²¹ð¾–RiîÏ°t/?/¸‰B -лùݽ¨°(3¨xð†½òìJvŒŽzYuOr¯ÎÓ—²€|âDóG&^8"q"z=Lt1ô{æ¼uʺ}ŒzQqOsÇã—7‰{×ñpü¡xv´S|èq0 ÉYâ•Ç"©S4ŠsADàÙ	y5J\B`'×)*kÁ6P‡>@»3<?
5ñúÐÚ
ìã`P¨*Ê¡¹`Ž
Œ$ðs#ÄÙR@^%¨¬B¶uáGœð®À7%¼_ÝW‡øÙUn$G#PŠÿc*ɑöØJ_C yuUW‹4øK®G cÖñm:œ6¸MÙ>=M†J‰G6ó]õ8ƈÃVWqOkû®Rq­Ô=æµRy­Ô|ã³ó ~ÀÐå,´ÃC#à˜Ùv"†÷9ð‰#±(p€,¤"EæË2ðÜC@`å6®Ââv·phܨfmw͛è$â,F9|~¿ÿ~Žñžêúyd›±ÅOÀ_üüýµô5"u¥þýïKƒGŽ²Ô-
=YMÕ¼"ê|¡ó¶¾iëbϽÁgrÖ'¡9‡z^hû›þŸuå&'H¼
¹ó8ˆ‹¯ˆš{7sȺÑy[ÿÚo'ƒ7oÅšÇ´Øíb×t®fýø/•o°MzåäF	¢Ízºb1£Ã"}0J`_Þ`³ÁV/®YX
'Ï ‰3ìÆϨ»E)ó5ë,X'pE™¤–o.(µ¨/\¢UYš¸
…tl«C—šCQ_8‹Á)yGD}«UH¼ÆCËñžVÜÛõKnsÑRª&Ÿ¨‹x'—Pyù
×Íbׅ櫇¡#bWˆl›{¡&MV™ˆ
ρD†pˆÑ–Фrñœâ¬«pòèË÷±s¤ŽLF$ÆR°oih¨¥ò'Š+%7mòÐD«²tIŒÁp³˜Õi	˜Oj‡‡Z¬^߯U•äß\;h#ß¿\…á}"äŸ_[/ÙyØpnÔÑ´ä=¨äŸ`[0/>ä5")ÏC)'*±•)éÉ}x†ÕÙ©­zp«®|üŠ¸^ͪþ"¥ô	­D莕Dç'ŒXʇ4ÉöÞW}jSR>ø^5Ñw£}Y«oÒe 9à‰òt'rÈÎ$ [0.>æÕ×å	ÍÒR¹î¬ôêѤÜ5ç'c$õñ"Çm]–«ÌóÑÓ[Ÿ.!x‡¾Ÿp;ÒéÒEÐlžýau.ÔHû
'Aëqk×u%ÄË@t€†Íf>xØC¡…Àý2às`Çï¾}?þKbÇg±b<;m´^ÌrsE¼M|#	ö¥²]›~z1'°ãÀŠ~›8rÁƽD݊ý˜ü^x­e-0ÚôWa~*HG	zéo®bg%('TÜÐØ+µ.Â'HÝÙ
endstream
endobj
44 0 obj
<</Filter[/FlateDecode]/Length 616>>stream
H‰dTMoÛ0½ðÐ%@¬®¾mm§dë†:4»Ffdgp²ý÷#EJ'³‹c'ï=>RrĦ®Œ³r­¦µvÂ8×À³ÕM˜åPaíc]­á-¦´ÇÔþÃ3˜NoXP›(èU,Ç 6MgÈu×Íèú§¸M~2;"ê!Á/ݹngôÒ;c!R%;û2£È"sžD%b,@	 ¹­¨![Œ×²ì))cÉ[¡áç]|¦dŒð׳Yø¼'iZÜDÀŸ}'èWtci;>'¤zŒp©]`$ºv.â	"€kCÂYîUс"$d	`æ³x.	š)-ß
kxOÊãqÛô†¬ä-S̈́'ƒÀ@àHè6e–ÖI1¾EÅԍk®ä%|Ù¤ù¾$y°pßid%bçº¤n>HZ%×Í5ß"!%y*ü¬ƒO"ì€êáš_ÎÀg±å™(Pé,oÇʸŽßâæ<o•k®ä9VÜðéZ—všY>+æÓÍÝb-:I¼ì'<+q®ƒÎé8‡H›xsëÊ)ú–þÏ$Ækd¤c]IñŒ/(ÿKÀTR"å\Û?Yká¶ø6ž=§œ'ò*¬‹¬î'/-´
.ç¹x¹_N§O»ÍiwûéM¼ÇÜ
üã´²
þVܯOÓn܊›Õj¹ÙüÙ?N=boÅ;D~ÀG]=®àwùÕ½<Œ?û·aº»ƒÄâ[¿¾Oýîu˜êj{ìÿ¢GT~CIl§áx:Lƒ8þ<œ1ƒ¤LX,ž>×Õ?q@æ
endstream
endobj
13 0 obj
<</Intent 21 0 R/Name(Layer 1)/Type/OCG/Usage 22 0 R>>
endobj
21 0 obj
[/View/Design]
endobj
22 0 obj
<</CreatorInfo<</Creator(Adobe Illustrator 16.0)/Subtype/Artwork>>>>
endobj
30 0 obj
[29 0 R]
endobj
45 0 obj
<</CreationDate(D:20180321110657Z)/Creator(MATLAB, The MathWorks, Inc. Version 8.1.0.604 \(R2013a\). Operating System: Microsoft Windows 7.)/ModDate(D:20180321112203-03'00')/Producer(Artifex Ghostscript 8.54)/Title(C:\\Users\\ARTUR\\AppData\\Local\\Temp\\tp4792015e_cbd9_429d_9b9c_601433acb843.ps)>>
endobj
xref
0 46
0000000002 65535 f
0000000016 00000 n
0000000005 00000 f
0000018277 00000 n
0000018328 00000 n
0000000006 00000 f
0000000007 00000 f
0000000008 00000 f
0000000009 00000 f
0000000010 00000 f
0000000011 00000 f
0000000000 00000 f
0000000162 00000 n
0000059033 00000 n
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000059104 00000 n
0000059135 00000 n
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000000000 00000 f
0000020488 00000 n
0000059220 00000 n
0000018678 00000 n
0000020788 00000 n
0000020675 00000 n
0000019575 00000 n
0000019926 00000 n
0000019974 00000 n
0000020559 00000 n
0000020590 00000 n
0000020862 00000 n
0000021070 00000 n
0000022120 00000 n
0000027503 00000 n
0000043469 00000 n
0000058345 00000 n
0000059245 00000 n
trailer
<</Size 46/Root 1 0 R/Info 45 0 R/ID[<8665A1A704355243F6D4137D529D164A><5F036756FBF0B643B3615AD279F6AE6C>]>>
startxref
59561
%%EOF

